LightCode: Light Analytical and Neural Codes for Channels with Feedback

The design of reliable and efficient codes for channels with feedback remains a longstanding challenge in communication theory. While significant improvements have been achieved by leveraging deep learning techniques, neural codes often suffer from high computational costs, a lack of interpretability, and limited practicality in resource-constrained settings. We focus on designing low-complexity coding schemes that are interpretable and more suitable for communication systems. We advance both analytical and neural codes. First, we demonstrate that PowerBlast, an analytical coding scheme inspired by Schalkwijk-Kailath (SK) and Gallager-Nakibo\u{g}lu (GN) schemes, achieves notable reliability improvements over both SK and GN schemes, outperforming neural codes in high signal-to-noise ratio (SNR) regions. Next, to enhance reliability in low-SNR regions, we propose LightCode, a lightweight neural code that achieves state-of-the-art reliability while using a fraction of memory and compute compared to existing deeplearning-based codes. Finally, we systematically analyze the learned codes, establishing connections between LightCode and PowerBlast, identifying components crucial for performance, and providing interpretation aided by linear regression analysis.

==> algo_sparse.tex <==
\section{Sparse Feedback Codes}\label{sec:algo_sparse}

We propose Sparse Feedback Code (SFC), a hybrid block feedback coding scheme that combines traditional feedback codes with deep-learning-based Joint Source Channel Codes (JSCC) to design novel block feedback codes. 

The key motivation behind a hybrid feedback coding scheme is the very poor forward channel experienced during the initial rounds of communication which makes use of any coding scheme undesirable. Hence, we propose using simple schemes such as SK during the initial rounds of communication and switching to deep-learning-based feedback schemes only for the later rounds of communication where the effective forward channel has effectively improved. Inspired by the two-phase strategy in \cite{gallager2009variations, anki2023isitcompressed}, we propose taking advantage of the discrete nature of the signal when the effective channel is improved. By computing the error vector of the estimated message, we can reduce the message to be transmitted to a discrete sparse vector and can formulate the problem as a JSCC of a sparse vector over AWGN channel. 

% \subsection{Revisiting Gallager's high SNR scheme}


% \subsection{List decoding version of Gallager's scheme}

\subsection{Joint Source Channel Coding of Sparse Vector}
Shannon's separation theorem \cite{shannon1948mathematical} states that at asymptotically large lengths, it is optimal to separately perform source and channel coding. But in practice, this does not hold well, especially when operating at short block lengths. Additionally, the lack of good source or channel codes at short block lengths increases the difficulty of the problem. To this extent, we propose using deep-learning-based JSCC approach to effectively solve this problem. This approach has proven effective in transmission of sources such as images over AWGN channels~\cite{choi2019neural,bourtsoulatze2019deep,kurka2020deepjscc}.




==> gbaf.tex <==
\section{Understanding GBAF}\label{sec:gbaf}
Introduced in~\cite{ozfatura2022all}, GBAF introduces the idea of block coding into the deep-learning-based feedback coding schemes. This is the key difference between GBAF and existing deep-learning schemes such as Deepcode~\cite{kim2018deepcode}, where to encoding of codeblock of $L$ bits is done by mapping all $L$ bits to one real-valued symbol and transmitting on the forward channel. The estimate of this symbol at the receiver is progressively improved in the next $L-1$ rounds with the help of feedback mechanism, resulting in a rate $\sfrac{1}{L}$ code. This is understandably impractical as the codeblock length $L$ grows, introducing large latency in the communication system. Hence, by limiting the rounds of communication to $D$, the message block of $L$ bits can be divided into blocks of size $K = \sfrac{L}{D}$. Operating on this principle, GBAF encodes the data in a two-dimensional fashion. Encoding is performed across the rounds by concatenating the message and feedback from previous rounds causally and using a series of feature extractors and multi layer perception (MLP) modules. Additionally, positional embedding and a self-attention based transformer encoder layer is deployed to encourage mixing of information across positions, introducing a block coding. Specifically, in~\cite{ozfatura2022all}, GBAF looks a block size $K=3$ and codeblock length of $L=51$ and performs a block coding across $17$ symbols. 

It is well known that the transformer architecture does not scale well to larger sequences. The self-attention mechanism imposes a compute complexity of $O(n^2)$ during training and $O(n)$ during inference, using KV cache, with respect to input length $n$. Further, a memory complexity of $O(n^2)$ prohibits from training the algorithm using a large batch size, which is crucial for attaining a good performance for any deep-learning models. 




tHence, we investigate the contribution of the self-attention mechanism to the performance of GBAF by performing an ablation study to better understating the compute vs performance trade-off.


% reference from GBAF JSAIT paper 
\begin{table}[!htp]
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{SNR (dB)} & \textbf{GBAF} & \textbf{GBAF (no attn, with PE)} & \textbf{GBAF (no attn, no PE)} \\
\midrule
-1.5 & 9.8e-5 & 7.5e-5 & 2.6e-5 \\
-1.0 & 2.6e-9 & 1.2e-9 & 2.7e-9 \\
0.0 & 5.4e-10 & 0.0 & 8e-10 \\

\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{Effect of self-attention on performance of GBAF. Ablation studies indicate that positional encoding and self-attention modules have no noticeable effect on the BLER performance.}
\label{tab:gbaf_ablation}
\end{table}

\prettyref{tab:gbaf_ablation} indicates a 


==> jsac/abstract.tex <==
% \section{Abstract}
\begin{abstract}\label{sec:abstract}
    %{\color{blue}To disucss: Title and the name for our coding scheme.}
    The design of reliable and efficient codes for channels with feedback remains a longstanding challenge in communication theory. %Existing theoretical schemes such as Schalkwijk-Kailath (SK) and \gn (GN) suffer from high latency and require high numerical precision as the blocklength increases. 
    While significant improvements have been achieved by leveraging deep learning techniques, neural codes often suffer from high computational costs, a lack of interpretability, and limited practicality in resource-constrained settings. %from high computational costs, lack interpretability, and are impractical for many present-day communication devices operating in resource-constrained settings. 
% 
    %Recent progress via deep learning techniques has shown promise but often comes with high computational costs and lack of interpretability, limiting practicality in resource-constrained settings.
    %
    We focus on designing low-complexity coding schemes that are interpretable and more suitable for communication systems. We advance both analytical and neural codes. First, we demonstrate that \pb, an analytical coding scheme inspired by Schalkwijk-Kailath (SK) and \gn (GN) schemes, achieves notable reliability improvements over both SK and GN schemes, outperforming neural codes in high signal-to-noise ratio (SNR) regions.
    Next, to enhance reliability in low-SNR regions, 
    we propose \lightcode, a lightweight neural code that achieves state-of-the-art reliability while using a fraction of memory and compute compared to existing deep-learning-based codes. Finally, we systematically analyze the learned codes, establishing connections between \lightcode and \pb, identifying components crucial for performance, and providing interpretation aided by linear regression analysis.
    %% Connect the two back. 
    
    % Further, the trade-off in complexity vs. performance for deep-learning-based feedback codes against classical schemes still remains unclear. In this work, we demonstrate the benefits of using simple classical feedback schemes in regions of sufficiently high-SNR and show that deep-learning-based codes can provide the highest gains in regions of low-SNR. 
    % Further, we propose a variation to \gn that noticeably improves the performance. 
    % Finally, we present \lightcode, a lightweight neural code for channels with passive feedback that achieves state-of-the-art block error rate performance while using a fraction of the parameters compared to current deep-learning-based solutions.
    
\end{abstract}



\begin{IEEEkeywords}
Channels with Feedback, Deep Learning, Channel Coding, Feedback Coding, Finite Block Length Coding
\end{IEEEkeywords}

% we present a two-phase approach that combines the classical feedback coding schemes with neural feedback schemes to significantly reduce the computational cost with marginal trade-off in performance.}

==> jsac/algo_sparse.tex <==
\section{Sparse Feedback Codes}\label{sec:algo_sparse}

We propose Sparse Feedback Code (SFC), a hybrid block feedback coding scheme that combines traditional feedback codes with deep-learning-based Joint Source Channel Codes (JSCC) to design novel block feedback codes. 

The key motivation behind a hybrid feedback coding scheme is the very poor forward channel experienced during the initial rounds of communication which makes use of any coding scheme undesirable. Hence, we propose using simple schemes such as SK during the initial rounds of communication and switching to deep-learning-based feedback schemes only for the later rounds of communication where the effective forward channel has effectively improved. Inspired by the two-phase strategy in \cite{gallager2009variations, anki2023isitcompressed}, we propose taking advantage of the discrete nature of the signal when the effective channel is improved. By computing the error vector of the estimated message, we can reduce the message to be transmitted to a discrete sparse vector and can formulate the problem as a JSCC of a sparse vector over AWGN channel. 

% \subsection{Revisiting Gallager's high SNR scheme}


% \subsection{List decoding version of Gallager's scheme}

\subsection{Joint Source Channel Coding of Sparse Vector}
Shannon's separation theorem \cite{shannon1948mathematical} states that at asymptotically large lengths, it is optimal to separately perform source and channel coding. But in practice, this does not hold well, especially when operating at short block lengths. Additionally, the lack of good source or channel codes at short block lengths increases the difficulty of the problem. To this extent, we propose using deep-learning-based JSCC approach to effectively solve this problem. This approach has proven effective in transmission of sources such as images over AWGN channels~\cite{choi2019neural,bourtsoulatze2019deep,kurka2020deepjscc}.




==> jsac/algorithm.tex <==
\section{Proposed neural coding scheme: \lightcode}\label{sec:deepcode}

%% {\color{blue}Begin with our goal: we aim to develop neural codes -- but limit ourselves to the per-symbol level codes. We want simpler codes. We want codes that are good for noiseless and noisy channels. ... }{\color{red}Updated }

Our goal is to design lightweight neural codes without the need for block coding \textit{i.e.,} we limit ourselves to symbol-by-symbol schemes suitable for both noiseless and noisy feedback settings. To this end, we design a lightweight deep-learning-based scheme with $10 \times$ fewer parameters compared to existing schemes. Surprisingly, this low-complex solution achieves a performance superior to current state-of-the-art deep-learning-based block-coding schemes. We now present the architecture and training choices crucial to achieving this new state-of-the-art BLER performance.  


% , and surprisingly, it matches the performance of GBAF. 

% One of the limitations of feedback coding schemes prior to GBAF is the inability to serve a variety of rates \textit{i.e.,} only rates of the form $\sfrac{1}{D}, D\in \mathbb{Z^+}$ are supported. In order to overcome this, instead of processing 1 bit at a time, we begin the coding scheme by processing a block of $K$ bits into 1 symbol. In the next $D-1$ rounds, we refine the noisy symbol at the receiver using the feedback. Since we are assuming passive feedback, decoding is done only at the end of $D$ rounds. By independently varying $K$ and $D$ any rate of the form $\sfrac{K}{D}$ where, $K,D \in \mathbb{Z^+}$ can be supported, making the scheme more flexible, while simultaneously reducing the overall latency of the communication by a factor of $K$. To enable a direct comparison with GBAF, we consider the case of $K=3$ in this section. 

% Additionally, we observed that this modulation step plays a crucial role in improving the decoding performance while simultaneously reducing the overall latency of the communication by a factor of $K$.


% . Further, we are interested in both noiseless as well as noisy feedback scenarios. 


% In this section, we introduce \lightcode, a lightweight neural coding scheme for channels with feedback. One of the limitations of existing feedback coding schemes is the inability to serve a variety of rates \textit{i.e.,} only rates of the form $\sfrac{1}{N}, N\in \mathbb{Z^+}$ are supported, which was also a major limitation in our original work Deepcode. In order to overcome this, we begin the coding scheme by introducing a introducing a modulation block in the algorithm to map $K$ bits to one symbol and then transmit this symbol using $N$ rounds of communication, where $N$ can be determined by the system requirements. This helps us in supporting any rate of the form $\sfrac{K}{N}, K,N \in \mathbb{Z^+}$, making the scheme much more flexible. For a fair comparison with GBAF, we consider $K=3$ in this work. Additionally, we observed that this modulation step plays a crucial role in improving the decoding performance while simultaneously reducing the overall latency of the communication by a factor of $K$. 


% of Deepcode by reducing the complexity of sequence-to-one modeling task across the rounds.


% was the high latency experienced by transmitting $K$ bits using $K$ rounds of communication. While this is acceptable while optimizing for total channel uses, this is impractical to deploy real systems. For instance, the blocklength considered in Deepcode $K=51$ requires $51$ rounds rounds of communication. Hence, we propose to reduce this latency by introducing a modulation block in the original Deepcode algorithm to map $K$ bits to one symbol and then transmit this symbol using $N$ rounds of communication, where $N$ can be determined by the system requirements. This step plays a crucial role in improving the performance of Deepcode by reducing the complexity of sequence-to-one modeling task across the rounds. For a fair comparison with GBAF, we consider $K=3$ in this work. 

\subsection{\lightcode: Architecture}\label{sec:arch} 
%%%% {\color{blue} I suggest a flow like this: we tried out our per-symbol NN architecture -- happens to be as good as GBAF. Then the ablation studies comes up -- actually they didn't need the positional encoding/transformer encoder either.} {\color{red} Updated}

% {\color{blue} Figure 3 right with the feature extractor in fig 4 and one layer MLP....}

% Our architecture. 

% Our architecture vs. RNN families. 
% Our architecture vs. GBAF codes. 

\textbf{Our architecture.} We split the design of the encoder-decoder architecture into two parts: the feature extractor and the multi-layer perception (MLP) module, as illustrated in~\figref{fig:simple_arch} (right). The choice of the feature extractor plays a crucial role in determining the downstream performance. A higher complexity feature extractor can perform better but might not be desirable for practical applications. For \lightcode, after experimenting with various choices, we found that the design illustrated in~\figref{fig:feature_extractor} gave the optimal trade-off in complexity vs. BLER performance.
% , \textcolor{blue}{the details of which are presented further}. 
% Specifically, we consider a hidden dimension of $d=32$ and 3 hidden layers. At the final layer, we use a skip connection to aggregate the outputs of layer 1 and layer 3 to project down to a latent dimension of $d=16$. The motivation for this architecture comes from our prior work on the design of deep-learning-based non-linear polar codes, \deeppolar~\cite{hebbar2024deeppolar}, where skip connections have proven crucial to ensure good performance. 
Further, the output of the feature extractor will be passed to an MLP module.
% to perform encoding or decoding. 
For the encoder, we choose a $1$ layer MLP to project the features to a $1$ dimensional output. For the decoder, we choose a $2$ layer MLP to transform the features into an output of dimension $2^K$. The full architecture for encoder and decoder, including the MLP are provided in~\appref{app:arch},~\figref{fig:encoder_decoder_arch}.

\medskip

\textbf{Our architecture vs. RNNs.} A popular choice for modeling the cross-round relation in feedback coding has been the RNN family of architectures. The sequential nature of the data makes it suitable for RNNs, GRUs, LSTMs, and other similar architectures. While these architectures provided impressive performance, a significant drawback is the necessity to store the hidden states from previous encoding steps, which is a high-dimensional latent that requires a lot of memory. Hence, a feed-forward architecture, which does not need a hidden state, is a better choice for resource-constrained scenarios. 

\medskip

\textbf{Our architecture vs. transformers.} While transformer models overcome the issue of storing hidden states by using positional encoding and self-attention, they also come with great computational complexity. Moreover, recent transformer-based feedback schemes proposed block coding using self-attention, which requires $O(n^2)$ memory and compute with respect to codeblock length. But as evident from results~\secref{sec:results}, block coding does not seem to provide noticeable gains in the setting under consideration. Hence, we propose a symbol-by-symbol coding scheme that uses a significantly simpler feed-forward architecture.

% \textcolor{blue}{In summary, the following are the key differences across the baseline architectures considered. DeepCode~\cite{kim2018deepcode} introduced the idea of using RNN architecture to model the dependencies across rounds and positions to design neural codes for channels with feedback. AttentionCode~\cite{shao2023attentioncode} improved this design by replacing RNNs with a more powerful sequence-to-sequence model, self-attention based transformer, to improve the modeling of temporal dependencies. GBAF~\cite{ozfatura2022all} improved this further by leveraging the transformer architecture to explicitly perform block coding across the bit positions and achieving the current state of the art in terms of BLER.}  

% \textcolor{blue}{In contrast to the existing {\color{red} existing neural schemes or existing transformer-based schemes} schemes that use a block length of $K=50$, \lightcode learns a code of length $K=3$. 

{\em Complexity.\ }By eliminating the need for block coding and using a short code length, \lightcode avoids the high-complexity transformer module used in GBAF architecture and instead uses a simple feed-forward network.
% also reduces the complexity of feature extractor by using the simple feed-forward network.} 
By carefully designing the architecture suitable for a symbol-by-symbol scheme, we achieve a lightweight design with more than $10\times$ reduction in the number of parameters compared to the RNN family of schemes such as Robust Coding and transformer family of block coding schemes such as GBAF. Further, we show in~\secref{sec:comp_throughput} that this reduction in complexity provides up to $171 \times$ higher decoding throughput compared to Robust Coding and up to $10\times$ higher throughput compared to GBAF. 
% {\color{red} I changed the order of this black part and the next paragraph. We don't want to write - complexity - training - complexity again. Revisit this paragraph - make it coherent and non-repetitive.} 

% {\color{red}DID YOU READ IT ONCE AGAIN? }




% thus reducing the complexity of the encoder-decoder, using simple feed-forward and skip connections as seen in~\figref{fig:feature_extractor}. Further, using a extremely large batch size of $5 \times 10^4$, \lightcode achieves a extremely low BLER and scales the performance to longer blocklengths by independently encoding a sub-block of 3 bits at a time, achieving superior performance compared to the state-of-the-art GBAF as seen from ~\figref{fig:bler_3_9_noiseless} and ~\figref{fig:bler_3_9_noiseless_51}.}

% We attribute this improvement to two factors. First is reduced complexity. As we considered a shorter code length, we were able to reduce the complexity of the encoder-decoder architecture by a factor of $10 \times $: \textcolor{blue}{By eliminating the transformer module used in GBAF for block coding and further reducing the complexity of feature extractor,}
% % {\color{brown} we removed a transformer...  and simplifies the feature extractor ... }
% using simple feed-forward and skip connections as seen in~\figref{fig:feature_extractor}. Second, the shorter code length and lightweight architecture allowed us to train \lightcode with an extremely large batch size of $10^5$, which is \textcolor{blue}{more than $10 \times$ larger than}
% % {\color{brown} how many times XX} times larger than 
% the maximum batch size suitable for GBAF codes. %whi


{\em Feature extractor.\ }{\figref{fig:feature_extractor} depicts the architecture of the feature extractor, which is the backbone for both encoder and decoder models. Compared to the feature extractor used in GBAF, we introduce two changes to improve the performance and reduce the complexity. The first is to add a skip connection, which preserves the prior from input to the feature extractor better, similar to the design of \deeppolar~\cite{hebbar2024deeppolar}. Further, the hidden dimension is reduced from $64$ to $32$, decreasing the number of parameters.}
% \textcolor{blue} {\color{red} somewhere highlight that the key difference is in the feature extractor, which is why we explain it next.} 
% The input is processed by three linear layers of dimension $32$ with two rectified linear unit (ReLU) activation functions in between. A skip connection is added in parallel to connect the output of the first layer to the final layer, which uses a hidden dimension of $32$, and the concatenated outputs are passed to the output layer, resulting in a $16$ dimensional feature space. % Two-level description is perferctly fine, but we do need to imply that this is a two-level description. So I used `specifically' blah blah. 

% Sure! This looks much better


Specifically, the input to the feature extractor is processed through a sequence of three linear layers, each with a hidden dimension of $32$, and rectified linear unit (ReLU) activation functions are applied between the first two layers. In parallel, we add a skip connection from output of first layer to input of final layer, which 
% to where? from input till right before the final layer? %, operating in parallel, 
reverses the sign of the representation to introduce variance in the information.  %<- What does this mean? to introduce variance in the information? Are there two skip connections? ``The first is to add a skip connection" OK Shall we put the two sentences on the skip connection together? 
% Currently skip connection -> dimension -> skip connection . Also, we have 'the first' but no 'the second' (or 'the other') So I guessed Further was the second part- but then when i saw 'skip connection' again, I wasn't sure whether there're two skip connections eg. 
%
% OK you wanted a two-level description? 
%
% Yes .. 
%
%
% Got it .. I used "Further" but Second is better. 
%
% And I initially described both changes .. and then started talking about the actual processing .. but makes sense to combine both
%
%
%
% Two changes: one skip connection, second is reducing dimension 
%
% In skip connection, instead of passing information as it is .. the sign is reversed. And the hypothesis is that, main connection already has the information .. by reversing the sign we are sort of changing the features.
These outputs are concatenated and passed through the final layer, which generates a 16-dimensional feature representation. %Probably we can comment this out? Skip connections are of course concatenated? Hmm are we describing the final layer by the way? Oh you mean the final layer generates a 16-dim feature representation OK. Looking good? great lets move on

% Yepp 


% Yes .. last statement needs to say something like " output from layer 3 is concatenated with the skip connection, and the final layer projects it to dim 16 feature" 
% Yes .. 


% , before passing to the final layer
% a feed-forward network with a hidden dimension of $32$, a sequence of linear layers and non-linear activation functions. A skip connection is added in parallel to connect the output of the first layer to the final layer, which uses a hidden dimension of $32$ and reverses the sign of the representation to introduce variance in the information. Finally, the output of the feature extractor is a $16$ dimension representation. To construct the encoder, a one-layer linear head is added to the feature extractor to project the feature vector from a dimension of $16$ to a $1$ dimensional output. Similarly, to construct the decoder, a two-layer linear head with an output dimension of $2^K$ is learned to project from a feature space of dimension $16$. } 
% {\color{red} Did you check typos? ``a output"!!!}


{\em Training.\ }Short code length and lightweight architecture allow for training of \lightcode with an extremely large batch size of $10^5$, which is more than $10 \times$ larger than the maximum batch size suitable for GBAF codes. We refer to~\secref{sec:training} for a detailed discussion of the training details and~\secref{sec:ablation} for an ablation study on the role of batch size.
% I added headers since we now discuss several sub-items.}

We now describe the detailed encoding and decoding procedure below.


% Our goal is to design lightweight neural networks while still achieving a competing performance. We consider a simple feedforward network for our encoder and decoder architecture, inspired by the \textit{feature extractor} and \textit{fully connected} modules from the GBAF architecture. We further simplify the design of the feature extractor design of GBAF by replacing a parallel processing pipeline with a simple skip connection, reducing the number of computations by half. In other words, our architecture is similar to %% In other words, we simplify 
% the architecture of GBAF after removing the complex modules supporting block coding and simplifying the feature extractor module, resulting in more than $10\times$ reduction in the number of parameters, as illustrated in \figref{fig:simple_arch}. %This is motivated by our observation from ~\prettyref{sec:gbaf} that block coding is adding little to no value for the BLER performance. % Again, we don't steal the thunder! 
% The encoding and decoding follow the procedure described in~\secref{sec:sysmodel}, described below. 

\medskip

\textbf{Encoding.} At round $i$, the encoder takes as input the original message and any available feedback from previous $i-1$ rounds to compute $x_i$. Further, after every round, a power reallocation is done across the rounds, similar to Deepcode~\cite{kim2018deepcode}. This is also based on the theoretical justification that allocating more power to the initial rounds results in an optimal performance~\cite{gallager2009variations}. The resulting encoding process at round $i$ is
\begin{equation}
    x_i = \alpha_i \phi(\mathbf{u}, \Tilde{y}_1, \Tilde{y}_2, \dots, \Tilde{y}_{i-1}, 0, \dots, 0),
\end{equation}
where $ \Tilde{y}_{i} = x_i + n_i + \Tilde{n}_i$ is the feedback from the previous round and $\alpha_i$ is the scaling factor to ensure sum power constraint across the rounds $\sum_{i=1}^D \alpha_i^2 = D$. Here, we note that in order to keep the size of the input to the encoder constant, the input is padded with zeros where necessary.

% {\color{blue} This paragraph is hard to follow.} {\color{red} Updated.}
% The input feature of dimension $K+D$, with the feedback from future rounds set to 0. 

\medskip

\textbf{Decoding.} At the end of $D$ rounds of transmission, the decoder uses all the received symbols and estimates the original message $\hat{\mathbf{u}}$ as
\begin{equation}
    \hat{\mathbf{u}} = \psi(y_1, y_2, \dots, y_D),
\end{equation}
where $y_i = x_i + n_i$ is the noisy received symbol in round $i$.

Here, $\phi$ and $\psi$ are the encoder and decoder neural networks based on the architecture in~\figref{fig:simple_arch}. Using this simple symbol-by-symbol scheme, \lightcode archives a performance similar to that of GBAF. It turns out that the computationally intensive self-attention mechanism and the cross-symbol coding are not adding considerable value to GBAF, as will be evidenced by our ablation studies in~\secref{sec:ablation}.

\medskip

\textbf{Choice of feature vectors.} Empirically, we observed that the choice of inputs to the feature extractor has a noticeable effect on the BLER performance based on the feedback channel. For noiseless feedback, the input features $(\mathbf{u}, y_1, y_2, \dots, y_i)$ worked the best. Further, as will be evident from discussions in~\secref{sec:noisy}, the input features  $(\mathbf{u}, x_1, x_2, \dots, x_i, n_1+\Tilde{n}_1, n_2+\Tilde{n}_2, \dots n_i+\Tilde{n}_i)$ gave the best performance for noisy feedback. Apart from this difference in features, the rest of the architecture remains the same for noiseless and noisy feedback scenarios. 
\begin{figure}[tb]
    \centering
 	\includegraphics[width=\linewidth]{figs/feature_extractor.pdf}
 	\captionsetup{font=small}
 	\caption{Feature extractor design for \lightcode for a rate $\sfrac{3}{9}$ code.}
    \label{fig:feature_extractor}
% \vspace{-1em}
\end{figure}

\medskip

\textbf{Support for multiple rates.} One of the limitations of existing symbol-by-symbol coding schemes is the inability to serve a variety of rates \textit{i.e.,} only rates of the form $\sfrac{1}{D}, D\in \mathbb{Z^+}$ are supported. In order to overcome this, instead of processing 1 bit at a time, \lightcode encodes a block of $K$ bits into $1$ symbol and communicates this symbol to the receiver over $D$ rounds. By independently varying $K$ and $D$ any rate of the form $\sfrac{K}{D}$ where, $K,D \in \mathbb{Z^+}$ can be supported, making the scheme more flexible, while simultaneously reducing the overall latency of the communication by a factor of $K$. The results for multiple rates for a block length of $K=3$ are discussed in~\tabref{tab:multi_rate}.


% In the next $D-1$ rounds, we refine the noisy symbol at the receiver using the feedback. Since we are assuming passive feedback, decoding is done only at the end of $D$ rounds. 



% The architecture of \lightcode can be adapted for any desired rate by controlling the number of rounds of communication $D$ as $R=\sfrac{K}{D}$. By changing the optimization objective in the loss function, we can tailor the code design based on the number of rounds of communication $D$, the results for which are discussed in~\tabref{tab:multi_rate}. Additionally, further rate control can be achieved by independently controlling the block length $K$. 


% The design of the feature extractor plays a crucial role in determining the downstream performance. A higher complexity feature extractor can provide a better performance but might not be desirable for practical applications. For \lightcode, after experimenting with various choices, we found that the design illustrated in~\figref{fig:feature_extractor} gave the optimal trade-off in complexity vs BLER performance. Specifically, we consider a hidden dimension of $d=32$ and 3 hidden layers. At the final layer, we use a skip connection to aggregate the outputs of layer 1 and layer 3 to project down to a latent dimension of $d=16$, which will be passed to the MLP module. The motivation for the architecture comes from our prior work on design of deep-learning-based non-linear polar codes, \deeppolar, where skip connections have proven to be crucial to ensure good performance~\cite{hebbar2024deeppolar}. 


% The input data is processed in two parallel streams that share the weights, but the data for the second stream is multiplied by -1. The motivation behind this design choice is that the flow on the top tackles the positive noise in the input while the flow on the bottom can tackle negative noise, and finally, the features are aggregated before projecting to the original feature dimension and passed to the MLP module for decoding.

% , while a transformer~\cite{vaswani2017attention} gave marginally better performance but a much higher complexity. 

% For \lightcode, after experimenting with various choices, we found that the design used in feature extractor \textit{(D)} in GBAF gave the optimal trade-off in complexity vs BLER performance, while a transformer~\cite{vaswani2017attention} gave marginally better performance but a much higher complexity. 

% The detailed architecture for the feature extractor module in~\figref{fig:simple_arch} is provided in~\figref{fig:feature_extractor}.
% Specifically, we consider a hidden dimension of $d=32$ and 3 hidden layers. The input data is processed in two parallel streams that share the weights, but the data for the second stream is multiplied by -1. The motivation behind this design choice is that the flow on the top tackles the positive noise in the input while the flow on the bottom can tackle negative noise, and finally, the features are aggregated before projecting to the original feature dimension and passed to the MLP module for decoding.










\subsection{Training}\label{sec:training}
Our primary region of interest is rate $\sfrac{3}{9}$ code at SNR $-1.0$ dB, where our target BLER is $\approx10^{-9}$. This is the current state-of-the-art performance by GBAF~\cite{ozfatura2022all}. To achieve such an extremely low error rate, it is important to train and simulate large amounts of samples reliably. Inspired by the high-SNR variant of \gn \cite{gallager2009variations}, we hypothesize that in regions of high-SNR or low errors, a significant benefit to the forward transmission arises from the power reallocation to symbols with non-zero errors. This can only be realized during the training by considering a large batch and enforcing the power constraint per batch.
Moreover, it is well understood that deep-learning models generalize better when trained with large batch sizes. Hence, we consider an extremely large batch size of $10^5$. While this is significantly larger than GBAF, which has a batch size of 8192, it is still a smaller number of symbols, considering that GBAF contains 17 symbols per codeblock. In contrast, our scheme consists of only $1$ symbol per codeblock. Further, it is possible to train with such a large batch size because of the small number of parameters compared to other deep-learning-based coding schemes. For a fair comparison, we follow a training methodology similar to that of GBAF, as explained below.  

\RestyleAlgo{ruled}

\SetKwComment{Comment}{/* }{ */}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\SetKwInput{KwData}{Data}
\SetKwInput{KwIn}{In}
\SetKwInput{KwOut}{Out}


\begin{algorithm}[hbt!]
\caption{Training \lightcode}
\label{alg:lightcode}


\KwInput{Encoder model $\phi$, Decoder model $\psi$, Block length $K$, number of rounds $D$,  forward noise variance $\sigma_{ff}^2$, feedback noise variance $\sigma_{fb}^2$, batch size $B$, number of epochs $E$, learning rate $\texttt{lr}$ }
\vspace{5pt}
\For{$i \leq E$}{
    \vspace{5pt}
    Generate batch of random binary vectors $\mathbf{u} \in \{0,1\}^{K \times B}$\\
    \vspace{5pt}
    % \Comment*[r]{Encoding over $D$ rounds}
    \For{$i \leq D$}{\Comment*[r]{Encoding at round $i$}
        \vspace{5pt}
        
        \If {$\sigma_{fb}^2 == 0$}{
            $x_i = \phi \left(\mathbf{u}, y_1, y_2, \dots, y_{i-1}, 0, \dots, 0 \right)$ }
        \vspace{5pt}
    
        \Else{
            $x_i = \phi \left(\mathbf{u}, x_1, \dots, x_i, n_1+\Tilde{n}_1, \dots n_i+\Tilde{n}_{i-1}, \dots, 0 \right)$ }
        $y_i = x_i + n_i$\vspace{5pt}} %\Comment*[r]{Transmission on forward channel} 
        
   $\mathbf{p_u} = \psi(y_1, y_2, \dots, y_D)$ \Comment*[r]{Decoding after $D$ rounds}
    \vspace{5pt}
    Compute the multi-class cross entropy loss $ \frac{1}{B} \sum_{j=1}^{B} \mathcal{L}_{\text{CE}}(\mathbf{c_j},\mathbf{p_{u_j}})$, $\mathbf{c_j}$ is the class index corresponding to $j^{\text{th}}$ message vector $\mathbf{u_j}$ and $\mathbf{p_{u_j}}$ is class probability vector after the \texttt{SoftMax} layer.\\
    \vspace{5pt}
    Clip the gradients to $0.5$.\\
    \vspace{5pt}
    Update model parameters for $\phi$ and $\psi$ using \texttt{AdamW} optimizer with learning rate \texttt{lr}.\\
    \vspace{5pt}
    Update the learning rate using \texttt{LambdaLR}. %scheduler.
}


\end{algorithm}


We use \texttt{AdamW} optimizer, a stochastic optimization method that modifies the typical implementation of weight decay in \texttt{Adam} by decoupling weight decay from the gradient update. We initialize the learning to $10^{-3}$ and use a \texttt{LambdaLR} scheduler with a weight decay of $0.01$. Additionally, we clip all the gradient values to $0.5$ for numerical stability. Starting with randomly initialized weights, we jointly train the encoder and decoder models on $1.2\times10^5$ batches. Each input symbol corresponds to $K$ bits, resulting in a $2^K$ category classification problem for the decoder. Accordingly, we use the multi-class cross entropy (CE) loss to measure the performance as
\begin{equation*}
    \mathcal{L}_{\text{CE}} = \frac{1}{B} \sum_{i=1}^{B} \left(  \sum_{j=0}^{2^K - 1}  c_{ij} \log p_{ij} \right),
\end{equation*}
where $B$ is the batch size, $2^K$ is the number of classes , $c_{ij}$ is the true class probability and $p_{ij}$ is the predicted probability of the $j^{\text{th}}$ class, for the $i^{\text{th}}$ sample.



% Accordingly, we use negative log-likelihood (NLL) loss to measure the performance as
% \begin{equation*}
%     L_{\text{NLL}} = -\frac{1}{B} \sum_{i=1}^{B} \left( y_i \times \log(p_{i, c_i}) + \sum_{j\neq c_i}^{K} \log(1 - p_{i, j}) \right).
% \end{equation*}
% \begin{equation*}
% \mathcal{L}(\theta) = -\frac{1}{N} \sum_{i=1}^{N} \log(p(y_i | x_i, \theta))
% \end{equation*}


The hyperparameters used for training the rate $R = \sfrac{3}{9}$ code are listed in~\tabref{tab:hyperparameters}.

\begin{table}[!ht]
\centering


\begin{tabular}{lc}
\hline
\textbf{Hyperparameter} & \textbf{Value} \\
\hline
Encoder training SNR & -1.0 dB \\
Decoder training SNR & -1.0 dB \\
Mini batch size ($B$) & 100,000 \\
Total epochs ($E$) & 120 \\
Batches per epoch & 1000 \\
Optimizer & AdamW \\
Initial learning rate ($\texttt{lr}$) & $10^{-3}$ \\
Learning rate scheduler & LambdaLR \\
\hline
\end{tabular}
\captionsetup{font=small}
\caption{Hyperparameters for training rate $\sfrac{3}{9}$ \lightcode. }
\label{tab:hyperparameters}
% \vspace{-1em}
\end{table}

Once the training is complete, we compute the mean power and standard deviation for the encoded data after every round for a large number of samples, $O(10^6)$, to reliably estimate the mean and standard deviation corresponding to encoder outputs to be used during inference. This is crucial in enforcing the power constraint in expectation. The algorithm for training \lightcode is described in detail in~\algref{alg:lightcode}.




% \begin{equation}
%     L_{\text{CE}} ( \hat{\mathbf{u}}, \mathbf{u}) = -\sum_{c=1}^{2^K}\log \left( \frac{\exp(W[i,c])}{\sum_{c=0}^{2m-1} \exp(W[i,c])} \right)

% \end{equation}


==> jsac/analysis.tex <==
\section{Analysis}\label{sec:analysis}
% 
% .{\color{blue} Add a wrapper paragraph }{\color{red} updated}

As evident from results in~\secref{sec:results}, symbol-by-symbol neural coding schemes such as \lightcode can achieve performance comparable to block coding schemes such as GBAF. Consequently, we examine GBAF and \lightcode in greater detail to systematically analyze their architecture, training process, and performance, with the aim of identifying the key factors contributing to their performance. Furthermore, we compare the memory and computational complexity of \lightcode with existing schemes to quantify the gains. Finally, we provide an interpretation of the encoded representations of \lightcode.

\subsection{Ablation studies on GBAF}\label{sec:ablation}

%{\color{blue} The paragraph coming next: it is stealing our thunder here. A better narrative will be -- we tried out a per-symbol coding scheme. Surprisingly, it matches the performance of GBAF! and present it in the next section. This section should end with several question marks only (no answers!).} {\color{red} Updated}
% 

We investigate the contribution of the self-attention mechanism to the performance of GBAF by performing an ablation study to understand the compute vs performance trade-off better. First, the self-attention mechanism is disabled, and it is observed that this has no significant effect on the BLER performance. Next, both self-attention and positional encoding blocks are disabled, and the performance remains approximately the same. These results, provided in~\tabref{tab:gbaf_ablation}, demonstrate a surprising observation that the self-attention and PE modules, which are responsible for cross-symbol block coding, contribute only marginally to the performance of GBAF. This brings into question the value of block encoding and motivates us to find simpler designs that perform only symbol-by-symbol coding while providing competing performance. 

% reference from GBAF JSAIT paper 
\begin{table}[!htp]
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{SNR (dB)} & \textbf{GBAF} & \textbf{GBAF (no attn)} & \textbf{GBAF (no attn, no PE)} \\
\midrule
-1.5 & 9.8e-5 & 7.5e-5 & 2.6e-5 \\
-1.0 & 2.6e-9 & 1.2e-9 & 2.7e-9 \\
 ~0.0 & 5.4e-10 & 6.6e-10 & 8.1e-10 \\

\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{Effect of block coding on performance of GBAF for rate $\sfrac{3}{9}$ code with noiseless feedback. Positional encoding and self-attention modules have no noticeable effect on BLER performance.}
\label{tab:gbaf_ablation}
\vspace{-1em}
\end{table}


\subsection{Scaling laws: batch size}\label{sec:scaling}
In section \secref{sec:results}, we have demonstrated that it is possible to achieve performance comparable to GBAF with fewer parameters and lower compute complexity. We also hypothesized in \secref{sec:training} that it is important to train the encoder using a very large batch size to accurately capture the statistics of the distribution so that the available power can be optimally allocated to the symbols with error at the receiver while reducing the power to the remaining symbols in a batch. In deep learning literature, it is well known that increasing the batch size can noticeably improve the performance of the neural network model~\cite{bahri2021explaining}. To better understand the effect of batch size on \lightcode, we perform a systematic study by training \lightcode with different batch sizes. As noted in \figref{fig:deepcode_scaling}, at a batch size of $1.5\times10^3$, \lightcode has a BLER of $3.7\times10^{-9}$, similar to that of GBAF (w/o BU). However, the BLER drops to $4\times10^{-10}$, outperforming GBAF when the batch size increases to $5\times10^4$ and beyond. We would like to note that for each batch size, hyperparameters such as learning rate have been optimized, and the model is trained until saturation to ensure the best possible performance.

\begin{remark} \textnormal{ Using a lightweight network with a small number of parameters makes it feasible to train with a very large batch size, resulting in a significantly lower error rate. }

\begin{figure}[!htb]
    \centering
 	\includegraphics[width=\linewidth]{figs/deepcode_scaling.pdf}
 	\captionsetup{font=small}
 	\caption{BLER performance of \lightcode with with respect to training batch size for rate $\sfrac{3}{9}$ code at SNR -1.0 dB with noiseless feedback. Performance improves significantly with respect to batch size, surpassing the performance of GBAF at batch size $ > 5\times 10^4$.}
 	\label{fig:deepcode_scaling}
% \vspace{-2em}
\end{figure}

\end{remark}

\subsection{Complexity and Throughput}\label{sec:comp_throughput}


We compare the total number of parameters in the encoder and decoder for a rate $\sfrac{3}{9}$ \lightcode against GBAF and Robust Coding within~\tabref{tab:num_params}. \lightcode reduces the parameter count by more than $10 \times$ compared to GBAF and Robust Coding, resulting in notable savings in memory.


\begin{table}[!ht]
\centering
\begin{tabular}{lc}
\hline
\textbf{Scheme} & \textbf{Total \# parameters} \\
\hline
GBAF~\cite{ozfatura2022all} & $9.1 \times 10^4$ \\
Robust Coding~\cite{kim2023robust} & $8.6 \times 10^4$ \\
\lightcode (ours) & $\mathbf{7.3 \times 10^3}$ \\

\hline
\end{tabular}
\captionsetup{font=small}
\caption{Rate $\sfrac{3}{9}$ \lightcode requires $< \sfrac{1}{10}^{\text{th}}$ the number of parameters compared to GBAF and Robust Coding.}
\label{tab:num_params}
\vspace{-1em}
\end{table}



\begin{table*}[!ht]
\centering

\begin{tabular}{lcccc}
\hline
\textbf{Scheme} & \textbf{ Enc (CPU)} & \textbf{ Dec (CPU)} & \textbf{ Enc (GPU)} & \textbf{ Dec (GPU)} \\
\hline
GBAF~\cite{ozfatura2022all} & $ 1.6 \times 10^5 $ & $ 1.7 \times 10^6 $ & $ 4.4 \times 10^8 $ & $ 3.3 \times 10^9 $\\

Robust Coding~\cite{kim2023robust} & $ 2.0 \times 10^5 $ & $  7.6 \times 10^4 $ & $ 4.1 \times 10^8 $ & $ 2.4 \times 10^9  $\\

\lightcode (ours) & $\mathbf{1.5 \times 10^6}$  & $\mathbf{1.3 \times 10^7 }$ & $\mathbf{2.9 \times 10^9}$  & $\mathbf{3.1 \times 10^{10} }$\\

\hline
\end{tabular}
\captionsetup{font=small}
\caption{Throughput (symbols/sec) comparison. Rate $\sfrac{3}{9}$ \lightcode achieves up to $ 10 \times $ higher decoding throughput compared to GBAF and up to $171 \times$ higher decoding throughput in CPU mode compared to Robust Coding.}
\label{tab:inference}
% \vspace{-1em}
\end{table*} 




% \begin{table}[!ht]
% \centering


% \begin{tabular}{lcc}
% \hline
% \textbf{Scheme} & \textbf{ Throughput (blocks/sec)} \\
% \hline
% GBAF~\cite{ozfatura2022all} & $ 2.9 \times 10^6 $ \\
% Robust Coding~\cite{kim2023robust} & $ 2.7 \times 10^6 $ \\
% \lightcode (ours) & $1.1 \times 10^7$  \\

% \hline
% \end{tabular}
% \captionsetup{font=small}
% \caption{Rate $\sfrac{3}{9}$ \lightcode achieves $ 4 \times $ higher throughput compared to GBAF and Robust Coding.}
% \end{table}\label{tab:inference}

% To compare the throughputs, we measure the inference time in CPU mode on a \texttt{Intel i9-9900X @ 3.50GHz} processor as well as in GPU mode using an \texttt{NVIDIA RTX 2080 Ti GPU}, using a batch size of $10^5$. \lightcode provides $10 \times$ higher throughput in CPU mode and $8 \times$ higher throughput in GPU mode compared to GBAF. Further, \lightcode provides up to $33 \times$ higher decoding throughput compared to Robust Coding in GPU mode, providing significant gains in latency, as shown in~\tabref{tab:inference}.



To compare the throughputs, we measure the inference time. We define the encoder throughput $T_E$ as the number of message blocks or symbols encoded per second and the decoder throughput $T_D$ as the number of message blocks or symbols decoded per second. Formally, for a rate $\sfrac{K}{D}$ code, the throughput can be defined as 
\begin{align}
    T_{EK} &= (\sfrac{K}{D}) T_E \hspace{2em} (\text{bits/sec}),\\ 
    T_{DK} &= (\sfrac{K}{D}) T_D \hspace{2em} (\text{bits/sec}).
\end{align}
We measure the throughput in CPU mode on a \texttt{AMD Ryzen Threadripper PRO 5975WX 32-Cores} processor and in GPU mode using an \texttt{NVIDIA GeForce RTX 4090}, using a batch size of $10^5 - 10^7$. \lightcode provides up to $10 \times$ higher encoding and decoding throughput than GBAF. Further, \lightcode provides up to $171 \times$ higher decoding throughput in CPU mode and up to $10 \times$ higher throughput in GPU mode compared to Robust Coding, providing significant gains in latency, as shown in~\tabref{tab:inference}.

We note here that comparing throughputs for classical schemes against deep learning-based schemes is not straightforward and depends heavily on the implementation. Our implementation of \lightcode uses \texttt{PyTorch} libraries, whereas \pb and other classical schemes were implemented using \texttt{NumPy} libraries. Further, a significant computational bottleneck for the classical schemes is the necessity for demodulation after each round, the speed of which is heavily influenced by the implementation methodology. Hence, we restrict our comparison to the family of deep learning codes, where the latency primarily originates from the architecture complexity and the total number of parameters, and a fair comparison is feasible. 
However, it is clear that the total number of numerical operations in classical schemes is significantly lower than that of deep-learning-based schemes, and we acknowledge that the throughput of classical schemes can be significantly higher.
% than that of any deep-learning-based schemes.}

\medskip

\textbf{Complexity vs. BLER trade-off:} While analytically quantifying the complexity of deep learning-based channel coding schemes with respect to target BLER would be very interesting, it is highly non-trivial and a widely open problem. Thus, we instead conduct an empirical study to analyze how the complexity of \lightcode scales with target BLER. Empirically, we observed that reducing the complexity of the decoder while maintaining the same complexity for the encoder provided the best trade-off in performance vs complexity. In this experiment, we vary the target BLER and empirically find the required encoder-decoder dimensions for a rate $\sfrac{3}{9}$ code at a forward SNR of $-1.0$ dB and a noiseless feedback channel. The results for the same are shown in~\tabref{tab:complexity}, demonstrating an almost linear degradation of BLER in log scale with the number of parameters.

\begin{table}[H]
\centering
\begin{tabular}{lccc}
\hline
\textbf{BLER} & Enc dimension & Dec dimension & \textbf{Total \# params} \\
\hline
$4.5 \times 10^{-10}$ & 32 & 32 &$7.3 \times 10^3$ \\
$3.4 \times 10^{-9}$ & 32 & 16 &$4.7 \times 10^3$ \\
$5.2 \times 10^{-9}$ & 32 & 12 &$4.3 \times 10^3$ \\
$2.8 \times 10^{-8}$ & 32 & 8 &$3.9 \times 10^3$ \\
% $\mathbf{1.3 \times 10^{-7}}$ & \textbf{16} & \textbf{32} &$\mathbf{5.9 \times 10^3}$ \\

\hline
\end{tabular}
\captionsetup{font=small}
\caption{Complexity vs BLER trade-off for rate $\sfrac{3}{9}$ code at a forward SNR of $-1.0$ dB and noiseless feedback. BLER (in log scale) degrades almost linearly with a decrease in the number of parameters.}\looseness=-1
\label{tab:complexity}
\end{table}

% {\color{red} \tabref{tab:complexity} should come here.}


% analytically quantifying the complexity of deep learning based channel coding schemes with respect to target BLER is non-trivial and an open problem. Hence we instead conduct an empirical study to analyze the trade-off in complexity vs performance of \lightcode. We observed that for $K=3$, decreasing the hidden dimension of encoder below $32$ is resulting in a significant drop in performance. Hence to reduce complexity, it is recommenced to reduce the hidden dimension of decoder, while marinating the same complexity for encoder. We provide the complexity vs performance trade-off for rate $\sfrac{3}{9}$ \lightcode with noiseless feedback at a forward SNR of $-1.0$ dB in~\tabref{tab:complexity}, which shows almost a linear degradation in BLER performance in log scale with respect to complexity of the decoder.}






% \begin{figure}[!htb]
%     \centering
%  	\includegraphics[width=\linewidth]{figs/complexity.jpg}
%  	\captionsetup{font=small}
%  	\caption{Complexity vs. BLER performance trade-off for rate $\sfrac{3}{9}$. Encoder complexity is maintained the same while decoder complexity is reduced to decrease the number of parameters. The change in BLER is almost linear in log scale with respect to the number of parameters.}
%  	\label{fig:bler_3_9_noisy}
% % \vspace{-1em}
% \end{figure}


% \begin{table*}[!ht]
% \centering

% \begin{tabular}{lcccc}
% \hline
% \textbf{Scheme} & \textbf{ Enc (CPU)} & \textbf{ Dec (CPU)} & \textbf{ Enc (GPU)} & \textbf{ Dec (GPU)} \\
% \hline
% GBAF~\cite{ozfatura2022all} & $ 9.2 \times 10^4 $ & $ 6.1 \times 10^5 $ & $ 1.8 \times 10^8 $ & $ 1.2 \times 10^9 $\\
% Robust Coding~\cite{kim2023robust} & $ 7.1 \times 10^4 $ & $  1.9 \times 10^5 $ & $ 5.7 \times 10^7 $ & $ 2.8 \times 10^8  $\\
% \lightcode (ours) & $\mathbf{8.8 \times 10^5}$  & $\mathbf{8.3 \times 10^6 }$ & $\mathbf{8.6 \times 10^8}$  & $\mathbf{9.4 \times 10^9 }$\\

% \hline
% \end{tabular}
% \captionsetup{font=small}
% \caption{Throughput (symbols/sec) comparison. Rate $\sfrac{3}{9}$ \lightcode achieves $ 8 $ to $10 \times $ higher throughput compared to GBAF and up to $33 \times$ higher throughput compared to Robust Coding.}
% \label{tab:inference}
% \end{table*} 






\subsection{Interpretation of \lightcode}\label{sec:interpret}
%{\color{blue}add a wrapper paragraph }{\color{red}updated}

By independently encoding sub-blocks of length $K=3$ and limiting to a symbol-by-symbol strategy, \lightcode allows for better interpretability and analysis of the learned encoder representations compared to block coding schemes such as GBAF. By analyzing the power allocation and relation between encoder output and feedback from previous rounds, we draw connections between \lightcode and \pb. %show that \lightcode can be viewed as a non-linear version of \pb.
\subsubsection{Power distribution}
A key contributing factor to the superior performance of \pb compared to SK is the discrete-symbol scheme in the final round of communication. In the high-SNR regime, we are only interested in the error in the PAM index of the decoded symbol with respect to the original symbol; this will result in a sparse distribution where most of the samples are 0. Thus, a majority of the available power is naturally allocated to the symbol locations with non-zero error. Surprisingly, we find similar behavior for \lightcode towards the final rounds of communication where the error is sparse. 

To test this hypothesis, we choose a moderately sparse error regime for ease of analysis. In~\figref{fig:power_dist}, we plot the power distribution of the encoder output in round $7$ for rate $\sfrac{3}{9}$ code at SNR $-1.0$ dB and noiseless feedback by randomly sampling $50$ symbols. On the X-axis, we see the sample number, and on the Y-axis, we plot the magnitude of error in the integer PAM index of the estimate after round $6$ and compare it against the magnitude of encoder output in round $7$. Note that a difference in index of 1 corresponds to a magnitude of 2 in the un-normalized PAM from Eqn.~\ref{eqn:pam}. It is evident from~\figref{fig:power_dist} that the highest power is allocated to the symbols with error in the estimate.

% compute the estimate of the message after round 6 and compare the magnitude of difference in PAM index against the encoder output in round 7 for rate $\sfrac{3}{9}$ code at SNR $-1.0$ dB and noiseless feedback. As illustrated in \figref{fig:power_dist}, the highest power is allocated to the symbols with error in the estimate. {\color{blue}describe the figure. In fig 9, we do blah and X axis is bla Y is blah... expanding this paragraph a little bit}

\begin{figure}[!htb]
    \centering
 	\includegraphics[width=\linewidth]{figs/power_dist.pdf}
 	\captionsetup{font=small}
 	\caption{\lightcode allocates more power to the symbols with error in estimate from the previous round, improving the overall probability of decoding.}
 	\label{fig:power_dist}
% \vspace{-1em}
\end{figure}

\begin{figure}[!htb]
    \centering
 	\includegraphics[width=\linewidth]{figs/n1_vs_x2.pdf}
 	\captionsetup{font=small}
 	\caption{Output of encoder in round 2 ($x_2$) shows that the encoder is directly compensating for the noise experienced in round 1 ($n_1$). }
 	\label{fig:n1_vs_p2}
% \vspace{-1em}
\end{figure}


\begin{figure*}[!htb]
    \centering
 	\includegraphics[width=\linewidth]{figs/linear_reg.png}
 	\captionsetup{font=small}
 	\caption{Comparison of linear approximation (Y-axis) vs true encoder output (X-axis). As the rounds progress, the linearity of the relation between encoder output and the feedback from previous rounds breaks, making it harder for analytical schemes to perform well.}
 	\label{fig:linear_reg}
% \vspace{-1em}
\end{figure*}

 \subsubsection{Interpreting the encoder} 
 In~\figref{fig:n1_vs_p2}, we plot the output of the encoder in round 2 with respect to the feedback in round 1. The encoder is approximately transmitting a linearly scaled version of noise from round 1. Interestingly, for the symbols on the boundary of the constellation embeddings, the encoder does not need to transmit any data when the noise favors the ground truth, unlike in the SK scheme, where all noise needs to be corrected. For instance, consider $\Theta_1$, mapped to the symbol at the boundary on the left, where a negative noise in round 1 is favored. And $\Theta_8$ is mapped to the symbol at the boundary on the right, where a positive noise in round 1 is favored. In such scenarios, the transmit power saved here can be reallocated to other symbols, improving the overall decoding error, which is only possible because of the non-linear activation functions.  





Visualization of the encoder output beyond round 2 is difficult as the number of inputs to the encoder increases linearly with the number of rounds of communication. Alternatively, we test the linear dependency between $x_{i+1}$ and $\{x_1, \dots, x_i, n_1, \dots, n_i\}$ by performing a linear regression as
\begin{equation}
    \hat{x}_{i+1} = \sum_{j=1}^{i} \alpha_j x_j + \beta_j n_j + c,
\end{equation}
where $\alpha_j$ and $\beta_j$ are regression coefficients and $c$ is the intercept found using \texttt{LinearRegression} toolbox in \texttt{sklearn} over $10^6$ samples. To make the analysis tractable, we build one linear regression model for each symbol in the PAM constellation. In~\figref{fig:linear_reg}, we plot the predicted output using linear regression vs. true encoder output when the input PAM symbol index is $\Theta=1$, for rounds $j=2$ to $9$. It is evident that as the round number increases, the relation becomes highly non-linear, and hence, classical schemes such as SK and GN as other linear schemes~\cite{chance2011concatenated,mishra2023linear} fail to model these dependencies. 

We note that recent results in~\cite{devroye2022interpreting,zhou2024interpreting} show the possibility of using post-hoc interpretability techniques to analyze the deep-learning-based codes and learn analytical approximations for the learned codes. Making progress in this direction is an interesting avenue for future work. %We aim to make progress in this direction in future work.}

% \begin{figure}[!htbp]

% \centerline{
% % \hspace{-0.1in}
% \subfigure[]
% {
%     \centering
%  	\includegraphics[width=0.5\linewidth]{figs/linear_reg_round_6.png}
%     % \caption{Rate $\sfrac{3}{6}$}
%  	\label{fig:linear_reg_round_6}
% }
% \hspace{-0.25in}
% \subfigure[]
% {
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/linear_reg_round_9.png}
%  	\label{fig:linear_reg_round_9}
%   }

%  \vspace{-0.5em}
%   }
%   \captionsetup{font=small}
%   \caption{ Temporary plots}
% % \vspace{-1.5em}
% \label{fig:linear_reg}
% \end{figure}



==> jsac/analytical.tex <==
\section{Analytical Coding Schemes for Channels with Noiseless Feedback}\label{sec:analytical}
% We begin by looking at the case of noiseless feedback \textit{i.e.,} $\sigma_{fb}^2 = 0$. 
% 
In this section, we review analytical coding schemes for channels with noiseless feedback \textit{i.e.,} $\sigma_{fb}^2 = 0$. We begin by reviewing the celebrated Schalkwijk-Kailath coding scheme~\cite{schalkwijk1966coding_p1}, one of the seminal works in coding for channels with noiseless feedback. We then review a less widely-known scheme by \gn~\cite{gallager2009variations}. This is similar to the SK scheme for the first $D-1$ rounds. Still, it deviates significantly in the last round, tailoring for the transmission of discrete messages, often significantly improving the performance in one round of communication. The \gn (GN) scheme is typically not considered as a baseline as it exhibits a worse error rate compared to SK in certain regions of SNR. However, in the next section, we introduce a novel analytical coding scheme, building on the SK and GN schemes. This new scheme achieves a significantly lower error rate than the SK or GN schemes and is often comparable to highly complex neural coding schemes in high-SNR regions, defying the conventional belief that neural coding schemes are much more reliable than analytical ones.

% but we demonstrate a simple modification to the GN scheme that can provide a non-trivial boost in performance. 
 
 % resulting in a lower bit error rate under finite-blocklength transmission regimes. 

 % Why are we reviewing these two here? 

 % This section serves two purposes. First, we revisit the existing classical SK and GN schemes, which should be considered a baseline for any neural coding schemes. Second, in the next section, we introduce a novel analytical coding scheme, building on the SK and GN schemes. This new scheme achieves a significantly lower error rate than either the SK or GN schemes and is often comparable to highly complex neural coding schemes in high-SNR regions, defying the conventional belief that neural coding schemes are much more reliable than analytical ones.


 
 % {\color{red} correct the tone: GN is worse than SK, but later, we demonstrate that a modification can ... }  
 
 % \gn scheme, which achieves a lower error rate than the SK scheme and should be considered a baseline for any neural coding schemes. 
 
 

%{\color{blue} Sth to think about: how about we put PowerBlast under ``Analytical coding" section? } 

\iffalse 
% a two-phase strategy developed 
It combines the strategy developed by Elias~\cite{Elias1956ChannelCapacity} for transmission of a Gaussian random variable on a channel with noiseless feedback, with a novel high-SNR strategy 
resulting in error probability that decreases with exponential \textit{order} that increases linearly with respect to the number of rounds of communication. 
\fi 

% Finally, we review the recent advances in coding for feedback channels using deep learning.

\subsection{Schalkwijk-Kailath coding scheme}
The SK scheme considers the problem of transmitting a fixed number of bits on an AWGN forward channel and a noiseless feedback channel. The transmission begins by mapping $K$ bits of information symbols to a single $2^{K}$-ary pulse-amplitude modulation (PAM) symbol $\Theta$ from the constellation
\begin{equation}
   \Theta \in \{ \pm 1 \eta, \pm 3 \eta, \dots, \pm (2^K -1) \eta\}, 
   \label{eqn:pam}
\end{equation}
where $\eta=\sqrt{\sfrac{3}{(2^{2K}-1})}$ is the scaling factor to ensure unit power normalization of the PAM constellation. Even though a block of information is transmitted since all the $K$ bits of information are mapped to one PAM symbol, the SK scheme at its core can be considered a symbol-by-symbol feedback scheme. We now describe the SK coding scheme in detail.

In the first round, the uncoded PAM symbol is transmitted after accounting for power constraint $P$ \textit{i.e.,} $x_1 = \sqrt{P} \Theta$ as
\begin{equation}
    y_1 = x_1 + n_1,
\end{equation}
where $n_1 \in \mathcal{N}(0,\sigma_{ff}^2)$ is the noise in the forward AWGN channel. The received symbol $y_1$ is then sent back to the transmitter noiselessly. For the second round, the transmitter first computes the receiver's estimate of the transmitted symbol based on $y_1$ as $\hat{\Theta}_1 = \frac{ \sqrt{P}y_1}{ P + \sigma^2_{ff}}$ using linear minimum mean-square error (LMMSE). 
% = \frac{ y_1}{\sqrt{P}}$ using minimum-variance unbiased estimator (MVUE). 
In the second round, after receiving $y_1$ as feedback, the transmitter sends the scaled version of the {\em error} in the LMMSE estimate from the previous round, i.e., $\epsilon_1= \hat{\Theta}_1 - \Theta$. This process continues for the remaining rounds. % The receiver sends $\hat{\Theta}_1$ as feedback to the transmitter via noiseless feedback channel. -- The receiver sends $y_1$ noiselessly. 
In other words, starting from round $i=2$, the goal of the transmitter is to transmit the error in estimate from the previous round, $\epsilon_{i-1} = \hat{\Theta}_{i-1} - \Theta$, after scaling appropriately to satisfy the power constraint. The complete algorithm is described in~\algref{alg:SK}.
% ~\ref{alg:SK}. 
% {\color{red} Algorithm 12???}
%{\color{blue} Add Error Analysis: It is shown that the SK scheme achieves the following error.... 
%} {\color{red}done}
%

\medskip

\noindent\textbf{Error analysis.\ } 
It is shown in~\cite{ben2017interactive} that the probability of error for rate $\sfrac{K}{D}$ SK scheme is given by
\begin{equation}
    p_{SK} =  2(1 - 2^{-K})Q\left(   \sqrt{ \frac{3S(1+S)^{D-1}}{2^{2K}-1}     }       \right),
\end{equation}
where $S$ denotes the SNR of the forward AWGN channel on a linear scale. Note that~\cite{ben2017interactive} assumes a minimum-variance unbiased estimator (MVUE) at the end of round $1$, $\hat{\Theta}_1 = \frac{y_1}{\sqrt{P}}$, for ease of analysis but it is sub-optimal in terms of error in the estimate after round 1.

% \RestyleAlgo{ruled}

% \SetKwComment{Comment}{/* }{ */}
% \SetKwInput{KwInput}{Input}
% \SetKwInput{KwOutput}{Output}
% \SetKwInput{KwData}{Data}
% \SetKwInput{KwIn}{In}
% \SetKwInput{KwOut}{Out}


% \begin{algorithm}[hbt!]
% \caption{Schalkwijk-Kailath (SK) coding scheme}
% \KwInput{Message symbol $\Theta$, number of rounds $D$, forward noise variance $\sigma_{ff}^2$ }

% \vspace{5pt}
% \textbf{Round 1:}\
% \textbf{Tx:} 
% Power normalization: $x_1 = \sqrt{P}\Theta$\;
% Forward channel: $y_1 = x_1 + n_1$\;
% % \textbf{Rx:} Unbiased estimate of transmit symbol $\hat{\Theta}_1 = \frac{\sqrt{P}y_1}{P + \sigma_{ff}^2};$ 
% \textbf{Rx:} Unbiased estimate of transmit symbol $\hat{\Theta}_1 = \frac{y_1}{\sqrt{P}};$ 

% \vspace{5pt}
% \texttt{/* Tx sends the error in estimate $\hat{\Theta}_1 - \Theta$ over the next $D-1$ rounds */} \\
% \vspace{5pt}

% \While{$2 \leq i \leq D$}{
%     \textbf{Tx:} Compute the error in estimate of previous round  ${\epsilon}_{i-1} = \hat{\Theta}_{i-1} - \Theta$ \;
%     Power normalization: $x_i = \frac{\sqrt{P}}{\sigma_{i-1}} {\epsilon}_{i-1}$, $\sigma^2_{i-1} = \mathbb{E}[\epsilon^2_{i-1}]$\;
%     Forward channel:  $y_{i} = x_{i} + n_{i}$\;
%     \textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\epsilon}_{i-1} = \frac{\sqrt{P}\sigma_{i-1}}{P + \sigma_{ff}^2} y_{i}$ \;
%     \vspace{5pt}
%     Update the estimate of $\Theta$ as: $\hat{\Theta}_i = \hat{\Theta}_{i-1} - \hat{\epsilon}_{i-1}$
% }
% \vspace{5pt}
% \textbf{Decoding}: Map $\hat{\Theta}_D$ to the closest symbol in the $2^K$ PAM constellation.
% \label{alg:SK}

% \end{algorithm}
% \vspace{-1em}


\RestyleAlgo{ruled}
\SetAlgoNlRelativeSize{-1}
\LinesNumbered
\SetKwComment{Comment}{/* }{ */}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\SetKwInput{KwData}{Data}
\SetKwInput{KwIn}{In}
\SetKwInput{KwOut}{Out}


\setcounter{algocf}{0} 


\begin{algorithm}[hbt!]
\caption{Schalkwijk-Kailath (SK) coding scheme}
\label{alg:SK}


\KwInput{Message symbol $\Theta$, number of rounds $D$, forward noise variance $\sigma_{ff}^2$ }

\vspace{5pt}
\textbf{Round 1:}\
\textbf{Tx:} 
Power normalization: $x_1 = \sqrt{P}\Theta$\;
Forward channel: $y_1 = x_1 + n_1$\;
% \textbf{Rx:} Unbiased estimate of transmit symbol $\hat{\Theta}_1 = \frac{\sqrt{P}y_1}{P + \sigma_{ff}^2};$ 
\textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\Theta}_1 = \frac{\sqrt{P}y_1}{P+\sigma^2_{ff}};$ 

\vspace{5pt}
\texttt{/* Tx communicates the error in estimate $\hat{\Theta}_1 - \Theta$ over the next $D-1$ rounds */} \\
\vspace{5pt}

\While{$2 \leq i \leq D$}{
    \textbf{Tx:} Compute the error in estimate of previous round  ${\epsilon}_{i-1} = \hat{\Theta}_{i-1} - \Theta$ \;
    Power normalization: $x_i = \frac{\sqrt{P}}{\sigma_{i-1}} {\epsilon}_{i-1}$, $\sigma^2_{i-1} = \mathbb{E}[\epsilon^2_{i-1}]$\;
    Forward channel:  $y_{i} = x_{i} + n_{i}$\;
    \textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\epsilon}_{i-1} = \frac{\sqrt{P}\sigma_{i-1}}{P + \sigma_{ff}^2} y_{i}$ \;
    \vspace{5pt}
    Update the estimate of $\Theta$ as: $\hat{\Theta}_i = \hat{\Theta}_{i-1} - \hat{\epsilon}_{i-1}$
}
\vspace{5pt}
\textbf{Decoding}: Map $\hat{\Theta}_D$ to the closest symbol in the $2^K$ PAM constellation.



\end{algorithm}
% \vspace{-1em}


% \begin{algorithm}
% \caption{Schalkwijk-Kailath (SK) coding scheme}
% \SetAlgoNlRelativeSize{-1}
% \SetAlgoNlRelativeSize{0}
% \SetNlSty{textbf}{(}{)}
% \SetNlSty{}{}{}
% \DontPrintSemicolon

% \textbf{Round 1:}\;
% \textbf{Tx:} Encode the message $\textbf{u} \in \{0,1\}^K$ to a $2^{K}$-ary PAM symbol $\Theta$ \;
% Power normalization: $x_1 = \sqrt{P}\Theta$\;
% Transmit: $y_1 = x_1 + n_1$\;
% \textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\Theta}_1 = \frac{y_1 P}{1+P}$ \;

% \vspace{5pt}
% \textbf{Round n(>1):}\;
% \textbf{Tx:} Compute the error in estimate of previous round  ${\epsilon}_{n-1} = \Theta - \hat{\Theta}_{n-1}$ \;
% Power normalization: $x_n = \frac{\sqrt{P}}{\sigma_n} {\epsilon}_{n-1}$, where $\sigma^2_n = \mathbb{E}[\epsilon^2_{n-1}]$\;
% Transmit:  $y_{n} = x_{n} + n_{n}$\;
% \textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\epsilon}_n = \frac{\sqrt{P}\sigma_n}{P + \sigma^2} y_{n+1}$ \;
% Update the estimate of $\Theta$ as: $\hat{\Theta}_n = \hat{\Theta}_{n-1} - \hat{\epsilon}_{n-1}$
% \vspace{5pt}
% \end{algorithm}\label{alg:SK}

\subsection{\gn coding scheme}

% HK: Since the title here is 'G-N', I would begin by saying sth about G-N and then introduce Elias. 
In~\cite{gallager2009variations}, \gn proposed a two-phase scheme that builds on the Elias scheme~\cite{Elias1956ChannelCapacity}, also closely related to the SK scheme. While the SK scheme considers the problem of transmitting a discrete symbol, Elias studied the problem of transmitting a Gaussian random variable $U \sim \mathcal{N}(0,\sigma^2)$. The strategy for forward and feedback transmissions is similar to SK, where a scaled version of the error in the LMMSE estimate is transmitted in every round $ I>1$. The main difference between the SK and Elias schemes lies in that the SK scheme aims to refine the message itself, while the Elias scheme aims to refine the estimate of noise added in the very first transmission. 



%In~\cite{gallager2009variations}, \gn proposed an alternative to the SK scheme by combining the transmission strategies of SK by describing SK in terms of Elias scheme and 

GN scheme operates in two phases and % combines the Elias scheme and a discrete-symbol scheme for the high-SNR region and operates in two phases.
% 
relies on the assumption that after a sufficiently large number of rounds of the Elias scheme, 
% what communication? Elias scheme/ correcting the noise 
the effective SNR for the forward channel shall be adequate for the noise variance to be considered small compared to the distance between the symbols in the PAM constellation. 
% 
In such a high-SNR regime, a strategy superior to the Elias scheme can be implemented by taking advantage of the discrete nature of the signal. Instead of transmitting the original error vector %{\color{blue} error vector or error}
with respect to $2^K$-ary PAM, %{\color{blue}a shifted version of the signal centered around the most recent estimate is transmitted}.
%
the integer difference between the PAM index of the estimate and the true PAM symbol is transmitted. 
We refer to this as {\em discrete-symbol} scheme. %In other words, the new signal is the integer difference in the PAM index of the estimate and the true PAM symbol. 
This method results in an error exponent that decreases with an exponential \textit{order}, which increases linearly with the number of rounds. For this work, we assume that the high-SNR region is realized in the final round of communication, which is valid according to the 2-phase strategy described in~\cite{gallager2009variations}.

We now describe the GN scheme in detail. % More specifically, t
The first round of GN is simply uncoded PAM, except for the power allocation. In~\cite{gallager2009variations}, it is shown the optimal power distribution across $D$ rounds is attained by choosing $P_1$ and $P_2$ such that $P_1 + (D-1)P_2 = DP$ and $P_1 = P_2 + 1$, $P_1$ is the power constraint in round 1 and $P_2$ is the power constraint in remaining rounds. Hence, the transmission in round 1 is given by
\begin{equation}
    y_1 = \sqrt{P_1}\Theta + n_1.
\end{equation}
For the remaining rounds, the goal of the transmitter is to communicate the noise $n_1$ to the receiver as in the Elias scheme, %. And this strategy is Elias % similar to SK,
%
where the LMMSE estimate at the receiver is improved iteratively, and a maximum likelihood (ML) detection is used at the end of $D-1$ rounds of communication to map the estimate to the original PAM constellation. 

Finally, for the last round, GN uses a discrete-symbol scheme suitable for the high-SNR region by transmitting the error in the PAM index $U$. We follow the assumption from~\cite{gallager2009variations} that the high-SNR region guarantees that $U \in \{-1, 0, 1\}$ with high probability.
In~\cite{gallager2009variations}, an ML decoder is used for the ease of analysis across multiple rounds of discrete symbol schemes, which is sub-optimal. However, since we assume only one round of the discrete-symbol scheme in this work, we assume a maximum-a-posteriori (MAP) decoder, which is optimal for the performance. Hence, the final round of GN can be viewed as MAP detection on a constellation $\{-1, 0, 1\}$ with probability distribution $\{\sfrac{p_{GN1}}{2}, 1 - p_{GN1}, \sfrac{p_{GN1}}{2}\}$,  $p_{GN1}$ is the probability of error after $D-1$ rounds. The complete algorithm is described in~\algref{alg:GN} in Appendix,~\secref{app:alg_gn}.

% ~\ref{alg:GN} 

%{\color{blue} Add Error Analysis: It is shown that the \gn scheme achieves the following error.... 
%} {\color{red}done}

\medskip

\noindent\textbf{Error analysis.\ } The probability of error for a rate $\sfrac{K}{D}$ \gn scheme can be computed in two phases. The first phase can be analyzed as one round of uncoded PAM followed by $D-2$ rounds of Elias scheme, for which it is shown in~\cite{gallager2009variations} that the probability of error is given by
\begin{equation}
    p_{GN1} =  2(1 - 2^{-K})  Q\left(   \sqrt{ \frac{3(1+S - \frac{1}{D-1})^{D-1}}{2^{2K}-1}     }       \right),
\end{equation}
where $S$ denotes the SNR of the forward AWGN channel on a linear scale.

In the second phase, which corresponds to the final round, the discrete integer difference between the PAM index of the decoded message $\hat{M}$  and the index of the true message $M$ is transmitted. Here, the message index 
$M \in \{0, 1, 2, \dots, 2^K-1\}$ is deterministic based on the transmitted symbol $ \Theta \in \{ \pm 1 \eta, \pm 3 \eta, \dots, \pm (2^K -1) \eta\}$ and can be computed using a predetermined mapping, where $\eta$ is the scaling factor to ensure unit power normalization.  Similarly, $\hat{M}$ corresponds to the message index whose corresponding symbol is closest to the estimated transmitted symbol $\hat{\Theta}$.
% {\color{red}decoding it - what is `it' here? Something along the line of ... $\hat{M}$ corresponds to the message index whose corresponding symbol is closest to the estimated transmitted symbol $\hat{\Theta}$ ?}

As the error in the $(\hat{M} - M)$ lies in $ \{-1, 0, 1\}$ with probability distribution $\{ \sfrac{p_{GN1}}{2}, 1 -  p_{GN1},  \sfrac{p_{GN1}}{2}\}$ based on the assumption from~\cite{gallager2009variations}, the probability of error in decoding using a MAP decoder can be computed as
\begin{equation}
            p_{GN} = 2(1-p_{GN1})Q \left( \gamma \sqrt{S} \right) + p_{GN1}Q \left( \left( \frac{1}{p_{GN1}} - \gamma\right) \sqrt{S} \right),
\end{equation}
% 
% The high-SNR regime implies that $(\hat{m} - m) \in \{-1, 0, 1\}$ with probability distribution $\{ \sfrac{p_{GN1}}{2}, 1 -  p_{GN1}, \sfrac{p_{GN1}}{2} \}$, with high probability. 
% \begin{equation}
%             p_{GN} = 2(1-p_{GN1})Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{GN1}}} \right) + p_{GN1}Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{GN1}}} \right),
% \end{equation}
where $S$ is the SNR of the forward AWGN channel on a linear scale, and $\gamma$ is the detection threshold given by
\begin{equation}
            \gamma = \frac{1}{2 \sqrt{p_{GN1}}} + \frac{\sqrt{p_{GN1}}}{S} \log \left( \frac{2(1-p_{GN1})}{p_{GN1}}  \right). 
\end{equation}
%$S$ is the SNR of the forward AWGN channel in linear scale.
% It is shown in~\cite{gallager1962low} that the probability of error for rate $\sfrac{K}{D}$ \gn scheme, where the final round of communication is the high-SNR scheme, is given by
% \begin{equation}
%     p_{SK} =  2(1 - 2^{-K})Q\left(   \sqrt{ \frac{3S.(1+S)^{D-1}}{2^{2K}-1}     }       \right),
% \end{equation}
% where $S$ is the SNR of the forward AWGN channel in linear scale.








% \subsection{A high SNR variant}
% The SK scheme improves the effective quality of the forward channel by iteratively refining the estimate at the receiver. One interesting observation made in~\cite{gallager2009variations} is that after sufficient number of rounds, the effective SNR of forward channel is sufficiently good such that the distance between PAM symbols is large compared to the standard deviation of noise. In such high-SNR regime, a strategy superior to SK can be implemented by taking advantage of the  discrete nature of the signal. Instead of transmitting the original error vector with respect to $2^K$-ary PAM, a shifted version of the signal centered around the most recent estimate is transmitted. In other words, the new signal is the difference in integer PAM index. This method results in error exponent that decreases with an exponential order which increases linearly with the number of rounds. 

==> jsac/bibilography.tex <==
\vspace{-.8em} 
 \medskip
 \small
 \bibliographystyle{IEEEtran}
 \bibliography{bibilography}

% \clearpage
\normalsize
% \input{Appendix}

==> jsac/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work, we address the problem of designing lightweight coding schemes for channels with feedback. First, we propose an analytical scheme, \pb, that can be viewed as a combination of Schalkwijk-Kailath and \gn schemes. Using a hybrid strategy and taking advantage of the discrete nature of the signal in the final round, \pb noticeably outperforms both SK and GN, providing a performance that competes with current deep learning schemes in regions of high-SNR. 

Next, we propose a lightweight deep-learning-based scheme, \lightcode, that can achieve state-of-the-art BLER performance while using less than $\sfrac{1}{10}^\text{th}$ the parameters and compute complexity compared to existing deep-learning-based schemes. By limiting to a symbol-by-symbol strategy and carefully designing the feature extractor using skip connections, combined with a training strategy that uses a very large batch size of $10^5$, \lightcode achieves a BLER up to $\sim 10^{-10}$. 

Additionally, with the help of systematic ablation studies, we have demonstrated that the self-attention module in the transformer-based GBAF code has very little effect on the BLER performance, demonstrating the limited benefit of block coding in this regime. 

Further, we interpret the \lightcode to show that power distribution in the sparse error regime of \lightcode is similar to that of \pb, where a majority of the available power is allocated to the symbols with error. Finally, we also perform a linear regression on the encoder outputs and the feedback from previous rounds. Our findings show that although the early stages of communication exhibit a linear relationship, it becomes non-linear towards the later stages, underscoring the importance of employing deep-learning-based non-linear coding techniques to attain optimal performance in regions of extremely low SNR.

\section*{Acknowledgment}
This work was partly supported by ARO Award W911NF2310062, ONR Award N000142412542, NSF Award CNS-2008824, and the 6G$@$UT center within the Wireless Networking and Communications Group (WNCG) at the University of Texas at Austin.

\newpage

==> jsac/gbaf.tex <==
\section{Understanding GBAF}\label{sec:gbaf}
Introduced in~\cite{ozfatura2022all}, GBAF introduces the idea of block coding into the deep-learning-based feedback coding schemes. This is the key difference between GBAF and existing deep-learning schemes such as Deepcode~\cite{kim2018deepcode}, where to encoding of codeblock of $L$ bits is done by mapping all $L$ bits to one real-valued symbol and transmitting on the forward channel. The estimate of this symbol at the receiver is progressively improved in the next $L-1$ rounds with the help of feedback mechanism, resulting in a rate $\sfrac{1}{L}$ code. This is understandably impractical as the codeblock length $L$ grows, introducing large latency in the communication system. Hence, by limiting the rounds of communication to $D$, the message block of $L$ bits can be divided into blocks of size $K = \sfrac{L}{D}$. Operating on this principle, GBAF encodes the data in a two-dimensional fashion. Encoding is performed across the rounds by concatenating the message and feedback from previous rounds causally and using a series of feature extractors and multi layer perception (MLP) modules. Additionally, positional embedding and a self-attention based transformer encoder layer is deployed to encourage mixing of information across positions, introducing a block coding. Specifically, in~\cite{ozfatura2022all}, GBAF looks a block size $K=3$ and codeblock length of $L=51$ and performs a block coding across $17$ symbols. 

It is well known that the transformer architecture does not scale well to larger sequences. The self-attention mechanism imposes a compute complexity of $O(n^2)$ during training and $O(n)$ during inference, using KV cache, with respect to input length $n$. Further, a memory complexity of $O(n^2)$ prohibits from training the algorithm using a large batch size, which is crucial for attaining a good performance for any deep-learning models. 




tHence, we investigate the contribution of the self-attention mechanism to the performance of GBAF by performing an ablation study to better understating the compute vs performance trade-off.


% reference from GBAF JSAIT paper 
\begin{table}[!htp]
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{SNR (dB)} & \textbf{GBAF} & \textbf{GBAF (no attn, with PE)} & \textbf{GBAF (no attn, no PE)} \\
\midrule
-1.5 & 9.8e-5 & 7.5e-5 & 2.6e-5 \\
-1.0 & 2.6e-9 & 1.2e-9 & 2.7e-9 \\
0.0 & 5.4e-10 & 0.0 & 8e-10 \\

\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{Effect of self-attention on performance of GBAF. Ablation studies indicate that positional encoding and self-attention modules have no noticeable effect on the BLER performance.}
\label{tab:gbaf_ablation}
\end{table}

\prettyref{tab:gbaf_ablation} indicates a 


==> jsac/intro.tex <==
\section{Introduction}\label{sec:intro}

\iffalse 
{\color{blue}
paragraph 1: Feedback plays a crucial role in modern communications. For example, arq and harq are used for communications. 

Paragraph 2: Shannon feedback channel; doubly exponential error decay. SK and GN Schemes are there. 

Paragraph 3: Recently it is shown that DL-based codes further improve the reliability upon the classical codes. 

Paragraph 4: DL-based ones; however, ... "While these ..."  
}
\fi 

%%%%% Feedback plays a crucial role in modern wireless communications. ARQ and Hybrid ARQ significantly improve the reliability of communications. %%Generalizing ARQ is also of recent interest~\cite{ankireddy2023compressed}. % compressed error hybrid ARQ (CE-HARQ) introduced a block coding scheme to optimize the number of rounds of communication in a noiseless block feedback setting. 


%Accordingly, linear symbol-by-symbol coding schemes for non-asymptotic settings were introduced by Chance and Love in~\cite{chance2011concatenated}, which were further improved by Mishra et al. in~\cite{mishra2023linear}. However, as we demonstrate in~\secref{sec:interpret}, this assumption of linearity severely limits the performance in later rounds of communication.
% Both the schemes assume a symbol-by-symbol unit delay feedback, making them impractical for practical applications similar to the SK scheme. 
% Recently, in~\cite{ankireddy2023compressed}, compressed error hybrid ARQ (CE-HARQ) introduced a block coding scheme to optimize the number of rounds of communication in a noiseless block feedback setting. However, CE-HARQ utilizes separate source and channel coding schemes, making it sub-optimal in the finite block-length regime, and also cannot scale well to low block lengths of $< 100$.


\iffalse
% The review
Recent technological advancements have resulted in an exponential growth in the number of connected devices that require constant communication with extremely high reliability and ultra-low latency. The future 6G communications are expected to have reliability higher than $99.9999999\%$, i.e., a Block Error Rate (BLER) less than $10^{-9}$~\cite{dang2020should,geraci2022will}. Furthermore, with the expected latencies to be less than $0.1$ ms, it is clear that block lengths that can be supported are far from being asymptotically large. This brings us to the question of channel coding schemes in the finite or short block length regime that can achieve ultra-reliable communication. 

Reliable transmission of information over noisy channels is a well-studied problem. Shannon demonstrated in his seminal paper that, for asymptotically large block lengths, it is possible to transmit information over a channel as long as the channel coding rate is less than the capacity of the underlying channel~\cite{shannon1948mathematical}. Over the years, many ingenious coding schemes have been developed that asymptotically approach the capacity of the channel, such as Reed-Muller~\cite{muller1954application}, Bose-Chaudhuri-Hocquenghem BCH)~\cite{bose1960class},  Low Density Parity Check (LDPC)~\cite{gallager1962low}, Turbo~\cite{berrou1996near}, and most recently the first provably capacity-achieving codes Polar Codes~\cite{arikan2009channel}. While these had a tremendous impact on the practical deployment of communication systems and wireless communications in particular, they have been designed and optimized for asymptotic settings and point-to-point Additive White Gaussian Noise (AWGN) channel model. With communication systems becoming increasingly large and complex, with multiple sources of interference and complex fading environments, these codes may not be sufficient to serve the tremendous needs and requirements of the future generation of communications. 

While designing codes for non-AWGN channels is a highly non-trivial problem, one such interesting scenario studied in this work is the problem of coding for channels with feedback. 
\fi 

% Open with Shannon and doubly exp decay .. current scheme limited to ARQ HARQ. 
% original analytical schemes .. but limited performance / not good w.r.t deep-learning schemes improve the performance but not interpretable. 


Shannon introduced the concept of feedback channel in~\cite{shannon1956zero}. In a channel with feedback, the transmitter \textit{cooperates} with the receiver to improve the probability of successful transmission by utilizing the \textit{feedback} from the receiver. % Symbol-by-symbol feedback refers to the scenario where the transmitter sends one symbol at a time, and the corresponding feedback is received the next time. On the other hand, a block feedback scenario refers to the setting where the transmitter sends a block of symbols, and the feedback corresponding to the entire block is received in the next time instance. 
In~\cite{shannon1956zero}, Shannon assumes a perfect {\em noiseless} feedback channel with {\em unit delay} and demonstrates that the availability of feedback at the transmitter does not change the capacity of the resultant forward channel for memoryless channels. Interestingly, while the capacity remains the same, significant improvements in error exponents can be achieved with the help of feedback. 

% Shannon also demonstrated that huge improvements in terms of error exponents can be achieved with the help of feedback. 

One of the seminal schemes in the noiseless feedback setting has been provided by Shalkwijk and Kailath in~\cite{schalkwijk1966coding_p1,schalkwijk1966coding_p2} (SK) using a simple linear encoding scheme resulting in a doubly exponential error exponent for finite block lengths. %%In the SK scheme, the transmitter begins the communication by mapping the entire message block of length $K$ to one symbol using a $2^K$-ary Pulse Amplitude Modulation (PAM) and refines the estimate of the symbol at the receiver iteratively by transmitting a scaled version of most recent error in the estimate in each round.  <- TMI at this point. 
In~\cite{gallager2009variations}, a two-phase variant of the SK scheme, which we refer to as \gn (GN), was discussed that can lead to further exponential decay of the error, provided a sufficiently good SNR is available for the forward channel. 
% While achieving impressive performance, SK and GN schemes suffer from numerical precision issues in practice as the message block length increases. 
%
% However, the performance guarantees of this scheme for a finite number of rounds, which is crucial for viable deployment in practice, is still an open problem. Additionally, all of these schemes need a perfectly noiseless feedback channel, which is impractical.
%% Later, an asymptotic scheme to transmit a single bit that can achieve almost zero error probability with minimal energy requirement was introduced in~\cite{polyanskiy2011minimum}.  
% 
The SK scheme has been enhanced in various ways. The Modulo-SK scheme~\cite{ben2017interactive} and schemes by Chance-Love~\cite{chance2011concatenated} and Mishra et al~\cite{mishra2023linear}, extends the SK scheme for noisy feedback, while compressed error correction (CEC)~\cite{ooi1998fast} and accumulative iterative code (AIC)~\cite{perotti2021accumulative} focus on reducing channel use through continuous error vector compression, using noiseless feedback.

% A notable extension of the SK scheme, which is suitable for noisy feedback scenarios, is Modulo-SK~\cite{ben2017interactive}. Another set of important schemes in this line of work is compressed error correction (CEC) by Ooi and Wornell~\cite{ooi1998fast} and, more recently, accumulative iterative code (AIC)~\cite{perotti2021accumulative}, which perform continuous and iterative compression of the error vector to minimize the total number of channel uses asymptotically. 

% talk about SK/GN -- insufficient performance to justify the delay 

While guaranteeing impressive error exponents, SK and other analytical coding schemes have not been adapted to practical communication systems, as the improvement in performance does not justify the cost incurred in terms of high-numerical precision, increase in the amount of feedback, and large number of rounds of communication. Because of this, analytical feedback coding schemes in practice are limited to automatic repeat request (ARQ) and hybrid-ARQ (HARQ) retransmission schemes, where the receiver provides simple one-bit feedback to indicate success (acknowledgment/ACK) or failure (negative acknowledgment/NACK). Extending ARQ to multi-bit feedback is an interesting research topic; for example, compressed error hybrid ARQ (CE-HARQ)~\cite{ankireddy2023compressed} and Griffin et al.~\cite{griffin2023code} propose using full feedback from the receiver to iteratively improve the error vector at the receiver.  

% optimize the number of rounds of communication in a noiseless block feedback setting using perfect feedback from the receiver.


%because of limitations such as the need for high numerical precision and an asymptotically large number of rounds of communication.
%Because of this, 
 % However, CE-HARQ utilizes separate source and channel coding schemes, making it sub-optimal in the finite block-length regime, and also cannot scale well to low block lengths of $< 100$.
%% However, the underlying channel coding schemes were not designed or optimized for transmission in the presence of feedback, making them sub-optimal. 

% While the capacity-achieving feedback coding schemes minimize the total channel uses, a more important metric in practice is the error rate achievable for a given maximum number of rounds of communication. 

%Because of the stringent latency requirements, a crucial metric in practice is the performance achieved in a finite number of rounds of communication \emph{i.e.,} the error rate achievable for a given maximum number of rounds of communication. 

%%% Accordingly, linear symbol-by-symbol coding schemes for non-asymptotic settings were introduced by Chance and Love in~\cite{chance2011concatenated}, which were further improved by Mishra et al. in~\cite{mishra2023linear}. However, as we demonstrate in~\secref{sec:interpret}, this assumption of linearity severely limits the performance in later rounds of communication.
% Both the schemes assume a symbol-by-symbol unit delay feedback, making them impractical for practical applications similar to the SK scheme. 


% In spite of the impressive theoretical guarantees, analytical coding schemes in practice are still limited to automatic repeat request (ARQ) and hybrid-ARQ (HARQ) retransmission schemes. In this setting, the receiver provides simple one-bit feedback to indicate success (acknowledgment/ACK) or failure (negative acknowledgment/NACK). However, the underlying channel coding schemes were not designed or optimized for transmission in the presence of feedback, making them sub-optimal. 

% The difficulty in adapting SK and other analytical coding schemes for practical communication systems can be attributed to the limitations, such as the requirement of unbounded amplitude and infinite numerical precision, making them impractical to implement in today's hardware systems. Moreover, the assumption of an asymptotically large number of rounds of communication is impossible to accommodate. While the capacity-achieving feedback coding schemes minimize the total channel uses, a more important metric in practice is the error rate achievable for a given maximum number of rounds of communication. Because of the stringent latency requirements, this is often finite and small. Accordingly, linear symbol-by-symbol coding schemes for non-asymptotic settings were introduced by Chance and Love in~\cite{chance2011concatenated}, which were further improved by Mishra et al. in~\cite{mishra2023linear}. However, as we demonstrate in~\secref{sec:interpret}, this assumption of linearity severely limits the performance in later rounds of communication.
% % Both the schemes assume a symbol-by-symbol unit delay feedback, making them impractical for practical applications similar to the SK scheme. 
% Recently, in~\cite{ankireddy2023compressed}, compressed error hybrid ARQ (CE-HARQ) introduced a block coding scheme to optimize the number of rounds of communication in a noiseless block feedback setting. However, CE-HARQ utilizes separate source and channel coding schemes, making it sub-optimal in the finite block-length regime, and also cannot scale well to low block lengths of $< 100$.\looseness=-1


\iffalse 
Limitations with existing work: 
- Complexity is high 
- Interpretation is vastly lacking due to the inherently complex neural code structure. 

What we do: 
- Reviewing the literature on neural feedback codes 
- Revisit GN scheme/develop new analytical schemes 
- Efficient and interpretable (?) neural codes? 
\fi 

% {\color{blue}first sentence - recent advances revive interest in coding for channels with feedback}
Recent advances in deep learning revived the interest in coding for channels with feedback by leveraging the expressive power~\cite{raghu2017expressive} of deep neural networks.
% enabled the creation of a new line of work in the area of channel coding by leveraging the expressive power~\cite{raghu2017expressive} of deep neural networks. 
Several works proposed deep learning approaches to improve the performance of channel codes, ranging from augmenting analytical decoders with learnable parameters~\cite{nachmani2016learning, nachmani2018deep, ankireddy2023interpreting, hebbar2022tinyturbo} to creating novel neural network architectures based neural encoders and decoders~\cite{hebbar2023crisp, hebbar2024deeppolar} and improving the code design using sequential models~\cite{li2021learning,ankireddy2024nested}. 
% 
For channels with feedback, deep learning techniques were used to design new encoding and decoding schemes that take advantage of the high-capacity feedback channel. Deepcode~\cite{kim2018deepcode} modeled both encoder and decoder functions as recurrent neural networks (RNNs) to process a bit stream in a sequential manner to directly minimize the end-to-end transmission error over an additive white Gaussian noise (AWGN) channel.
% To overcome the limitations of the analytical feedback codes, deep-learning aided non-linear feedback codes were introduced by Kim et al. in Deepcode~\cite{kim2018deepcode}. 
Several works further explored this idea of using learning-based approaches for modeling the encoding and decoding operations, which can be broadly classified into the RNN family of codes~\cite{safavi2021deep,mashhadi2021drf,kim2023robust} and the transformer family of codes~\cite{shao2023attentioncode,ozfatura2022all}, discussed in detail in~\secref{sec:neural_codes}. The current state-of-the-art is generalized block attention feedback (GBAF)~\cite{ozfatura2022all}, which uses self-attention and transformer architecture to perform block coding. 


% Using non-linear encoders and decoders based on recurrent neural network (RNN) architecture, Deepcode outperforms both practical (numerically stable) SK and chance-love schemes. Deepcode overcomes the limitation of necessity for infinite precision by SK, and also, the encoded representations are within a finite power range. This demonstrated the existence of non-linear codes designed via deep learning techniques for complex channels that are not Additive White Gaussian Noise (AWGN) channels, such as feedback channels. Following the success of Deepcode, several works improved the results with a combination of various novel architectures and training methodologies. deep extended feedback (DEF) codes~\cite{safavi2021deep} improve the Deepcode by encoding over longer sequences to improve error correction and use higher-order modulation to improve the spectral efficiency. Deep Extended and deep SNR-robust feedback (DRF) codes~\cite{mashhadi2021drf} use a bi-directional long short-term memory (LSTM) network-based encoder and decoder architecture to design codes for fading channels. An SNR-aware attention mechanism was used to enable decoding at multiple SNR levels using a single model.  More recently, AttentionCode~\cite{shao2023attentioncode} was introduced based on a variant of the highly powerful self-attention based transformer architecture. Various training methodologies such as distributed learning and curriculum learning have been deployed, along with training on very large batch size, to achieve a BLER of up to $10^{-7}$ at SNR 0 dB for the rate of $\frac{3}{9}$. This was further improved in generalized block attention feedback (GBAF)~\cite{ozfatura2022all} that improves the BLER performance while reducing the communication overhead by employing block encoding and providing support for multiple rates. Moreover, GBAF performs block encoding to reduce the total rounds of communication needed to complete the transmission, making the latency suitable for These are the current state-of-the-art (SOTA) results in coding for channels with passive feedback, providing a magnitude of BLER performance gains over existing analytical feedback codes as well as Deepcode and other prior deep learning based feedback codes. Recently, GBAF has also been extended for the scenario of active feedback in~\cite{ozfatura2022feedback}.

% Our contrinbutions - the agenda
While these state-of-the-art deep-learning-based feedback codes provide tremendous improvements in BLER performance, they also come with significant memory and computational costs that may not be supported by the next generation of communication transceivers that operate with limited onboard resources. Therefore, it is desirable to develop lightweight codes that use simple schemes while providing desirable performance. To accomplish a reduced complexity coding scheme, we explore two different directions in this work. First, we review and understand the existing analytical feedback coding schemes to identify the limitations and propose a new feedback coding scheme that provides non-trivial performance improvements over the existing schemes for channels with passive, noiseless feedback. Next, we propose a lightweight deep-learning-based feedback coding scheme that can significantly reduce the complexity compared to neural block-feedback coding schemes by limiting ourselves to a symbol-by-symbol scheme instead of block coding schemes. 

% On the other hand, human-crafted schemes such as SK are extremely simple but have limited relevance in practice because of the large latency and numerical precision requirements. 

 

% In this work, we closely study GBAF, the current state-of-the-art feedback coding scheme for channels with noiseless feedback. By analyzing the architecture and the block encoding procedure, we propose modifications and simplify the scheme to perform symbol-by-symbol coding to greatly reduce the complexity. 

Our main contributions are summarized as follows:

%{\color{blue} In the bullets below, I would suggest adding references to the sections (Section X), (Section Y) to help readers navigate. }{\color{red} updated}
\begin{itemize}
    \item We provide a comprehensive review of the existing analytical and deep-learning-based coding schemes for channels with feedback and identify the limitations of existing approaches (\secref{sec:analytical} and \secref{sec:neural_codes}).
    
    % propose improvements to bring these schemes closer to practice. 
    
    \item We propose \pb, an analytical coding scheme that noticeably improves the performance over Schalkwijk-Kailath and two-phase \gn schemes (\secref{sec:pb}) and exhibits reliability comparable to state-of-the-art deep-learning-based coding schemes in regions of high-SNR (\secref{sec:results}).
    
    % which is an improvement to the classical 2-phase \gn \cite{gallager2009variations} scheme to noticeably boost the performance (\secref{sec:pb}) and demonstrate its gains (\secref{sec:results}).
    % and compare against GBAF, the current state-of-the-art for channels with feedback.

    % \item We investigate the performance of GBAF and demonstrate that block coding is not beneficial in the regime of interest
    % and does not scale well.  
    
    \item We propose \lightcode, a lightweight neural coding scheme that achieves a performance superior to current state-of-the-art feedback coding schemes using $10 \times$ fewer parameters and computational complexity (\secref{sec:deepcode}, \secref{sec:results}), while maintaining interpretability. 
    % {\color{blue} 10x reduction + analyzable }

    \item We analyze the representations learned by the \lightcode encoder using linear regression and draw comparisons with \pb. We also demonstrate that the relation between encoded symbols and the feedback is highly non-linear in the final rounds, underscoring the need for a deep-learning-based coding scheme (\secref{sec:analysis}).
    
    
    % to find analytical approximations that can provide ultra-lightweight encoding schemes, offloading the compute burden to the receiver. 

\end{itemize}


% Therefore it is desirable to explore the possibility of a reduction in computation complexity by combining analytical schemes with deep learning based schemes. Moreover, the effective SNR in the initial rounds of communication is very poor and it is hard for any coding scheme to provide meaningful improvement in performance. Inspired by the high-SNR scheme in~\cite{gallager2009variations}, we categorize the coding \textit{region} can be divided into low-SNR region where the noise power is comparable to the distance between any constellation symbols and high-SNR region where the noise variance is much smaller than the distance between adjacent constellation symbols. It was shown in~\cite{gallager2009variations} that significant improvement over SK scheme can be achieved in high-SNR region by taking advantage of the discrete nature of the signal. Accordingly, we propose that a analytical scheme is sufficient to achieve adequate performance in the low-SNR region, post which, in the high-SNR region, deep learning based schemes can be used to improve the performance significantly. Additionally, we leverage the sparsity of the error vector in the so-called high-SNR region to achieve a superior error correction performance by formulating the problem as a joint source channel coding (JSCC) problem.

% Our main contributions are summarized as follows:

% \begin{itemize}
%     \item We revisit the high-SNR variant of SK scheme by Gallager~\cite{gallager2009variations} to construct a scheme that achieves theoretical performance comparable to SOTA deep learning scheme
%     \item We propose a hybrid coding scheme, Sparse Block Feedback Code, that efficiently combines the classical SK scheme with recent deep learning based JSCC schemes to provide a performance comparable to SOTA deep learning based feedback coding schemes.
% \end{itemize}


% , impressive advancements have been made over the years using human-crafted codes and more recently using deep learning.  






% \begin{itemize}
%     \item Revisit Gallager scheme; propose a list decoding version 
%     \item We present SparseCode, a {\em hybrid} block feedback scheme that combines classical SK feedback scheme with novel Deep Learning based non-linear codes that leverage the sparsity in input vectors. By leveraging domain knowledge, we simplify the encoder-decoder design to use SK during the initial rounds of communication and switch to deep learning based communication only when the residual error is sparse, making the overall scheme more efficient.
%     \item Within the sparse error regime, we show that the gain achieved by SparseCode increases as the error improves with the sparsity as well as the block length.
%     \item Finally, we compare the performance of SparseCode with SOTA DL based feedback codes to demonstrate superior error correction performance in many regimes of interest.
%     \item (potentially) soft input
%     % Channels with noisy feedback; beyond AWGN channels; beyond bits
    
% \end{itemize}

==> jsac/neural_fb_codes.tex <==
\section{Deep Learning based Coding schemes}\label{sec:neural_codes}
% So far we have reviewed analytical coding schemes for channels with noiseless feedback and also proposed a variant of \gn. 

% Despite the impressive gains of \pb over \gn scheme, the performance can still be significantly worse compared to the deep-learning-based coding schemes in some regions. 

In this section, we review the current state of the learning-based codes for channels with feedback, closely analyze the generalized block attention feedback (GBAF)~\cite{ozfatura2022all}, discuss the shortcomings, and provide motivation for a new learning-based coding scheme we introduce in the next section.   

%% Should we make this section a little more comprehensive overview of learning-based codes? 


\subsection{RNN families}
% {\color{blue} Deepcode and Robust Coding? }

Deep-learning-based algorithms are capable of modeling complex input-output relations. One of the critical challenges in designing codes for channels with feedback is accurately computing the subsequent transmission that minimizes the probability of decoding error, conditioned on the feedback from previous rounds. Existing classical coding schemes employ linear estimators at the receivers and model the dependencies in a linear fashion at the transmitter, which is sub-optimal. Instead, the sequential nature of the feedback from previous can be better leveraged by using deep-learning architectures such as RNNs tailored for processing sequential data. Deepcode~\cite{kim2018deepcode} demonstrated this advantage in modeling the dependencies across bits and rounds using bi-directional gated recurrent units (GRUs). Several follow-up works investigated the use of other RNN-based architectures such as long short-term memory  (LSTMs)~\cite{safavi2021deep,mashhadi2021drf} and, more recently, Robust Coding~\cite{kim2023robust} was proposed, which combined attention mechanism with bi-directional GRUs to optimize the symbol-by-symbol code design for noisy feedback channels across the rounds. Despite the promising performance, one disadvantage of using RNN-based architecture is the necessity to store the hidden states of the model, which are typically of much higher dimensions than the inputs and demand a lot of memory. Additionally, the sequential and iterative nature of encoding and decoding in RNNs can result in significant latency in the system.

% Several followup works investigated various architectures such as RNNs, LSTMs, and attention-based mechanisms for solving this problem of encoding and decoding the data across the rounds. Interestingly, GBAF introduced another dimension of coding where a block of symbols were encoded across the codeword, in addition to coding across the rounds resulting in a magnitude of orders of magnitude improvement in performance at extremely low SNRs, albeit a heavy computational cost.

\begin{figure*}[!htb]
    \centering
 	\includegraphics[width=0.9\linewidth]{figs/simple_arch.pdf}
 	\captionsetup{font=small}
 	\caption{
    (Left)Architecture for GBAF: The positional encoding and transformer encoding modules are used for block coding to encourage the mixing of symbols across the positions. (Right): Using a symbol-by-symbol scheme, \lightcode significantly reduces the complexity of encoding and achieves more than $10$x reduction in the number of parameters. On the left, we see the architecture for GBAF~\cite{ozfatura2022all}, and on the right, we see the architecture for \lightcode (ours). }
    \label{fig:simple_arch}
\vspace{-1em}
\end{figure*}


\subsection{Transformer families}\label{sec:gbaf}
In another line of work, self-attention-based transformer architectures have been explored for designing neural feedback codes. AttentionCode~\cite{shao2023attentioncode} introduced the idea of replacing RNN-based architecture with pure attention-based models, resulting in better alignment between a symbol and the corresponding feedback. In other words, AttentionCode can be viewed as Deepcode with transformer architecture. By leveraging the attention mechanism, AttentionCode creates temporal correlations at the transmitter
for encoding and exploits these temporal correlations
at the receiver for decoding. Further, the inputs to the encoder and decoder transformers are restructured to align each bit with the corresponding noise from multiple rounds as a single column, processed by the self-attention mechanism. More recently, GBAF~\cite{ozfatura2022all} introduced the idea of performing block coding across the codeblock, in addition to temporal coding across the rounds, resulting in orders of magnitude improvement in performance at extremely low SNRs, explained in detail below. 

As illustrated in \figref{fig:simple_arch}, the encoding of GBAF is performed across the rounds by causally concatenating the message and feedback symbols from previous rounds and using a series of feature extractors and multi-layer perception (MLP) modules. Additionally, positional encoding (PE) and a self-attention-based transformer encoder layer are deployed to encourage the mixing of information across the symbols within a codeblock, leading to block coding. 
% 
More specifically, a block of $L$ bits is divided into $l$ sub-blocks of $K$ bits each and first encoded independently using a feature extractor. Next, PE and transformer encoder modules perform cross-symbol coding across the $l$ symbols. Finally, an MLP module is used to encode each symbol. A similar architecture is used at the decoder, but the output dimensions are adjusted accordingly. 

For concreteness, in~\cite{ozfatura2022all}, GBAF considers a block size $K=3$ and codeblock length of $L=51$ and performs a block coding across $l = 17$ symbols. This is the present state-of-the-art in performance, achieving a BLER of $7 \times 10^{-10}$ at SNR $-1.0$ dB for rate $\sfrac{3}{9}$.

% {\color{brown}Reads better. Let's align the description and Figure 3 closely -- what's little l in the figure? what's u? where is the feedback in Figure 3?} 
% {\color{red} Updated -- OK I found what's missing; we're missing how the encoding occurs over time. Figure 3 does not show feedback signals. It's showing how L bits are grouped instead. Also, we can add dimensions to clarify the description better.}



% In contrast, Robust Coding performs only coding across the rounds using GRUs



% Introduced in~\cite{ozfatura2022all}, GBAF introduces the idea of block coding into the deep-learning-based feedback coding schemes, which is the key difference between GBAF and existing deep-learning schemes such as Robust Coding~\cite{kim2023robust}. Deepcode maps 

% where to encoding of codeblock of $L$ bits is done by mapping all $L$ bits to one real-valued symbol and transmitting on the forward channel. The estimate of this symbol at the receiver is progressively improved in the next $L-1$ rounds with the help of feedback mechanism, resulting in a rate $\sfrac{1}{L}$ code. This is understandably impractical as the codeblock length $L$ grows, introducing large latency in the communication system. Hence, by limiting the rounds of communication to $D$, the message block of $L$ bits can be divided into blocks of size $K = \sfrac{L}{D}$. Operating on this principle, GBAF encodes the data in a two-dimensional fashion. Encoding is performed across the rounds by concatenating the message and feedback from previous rounds causally and using a series of feature extractors and multi layer perception (MLP) modules. Additionally, positional encoding (PE) and a self-attention based transformer encoder layer is deployed to encourage mixing of information across positions, introducing a block coding. Specifically, in~\cite{ozfatura2022all}, GBAF looks a block size $K=3$ and codeblock length of $L=51$ and performs a block coding across $17$ symbols. 

%{\color{blue} The description of GBAF is a little hard to follow.} %{\color{red} Updated}




\subsection{Important open problems} %Limitations of deep learning-based codes} % GBAF}


% {\color{blue}Let's end this section with a bunch of open problems: eg is across-symbol coding necessary? complexity can be further reduced? interpretation??} {\color{red} Updated}


While providing impressive performance and reliability, transformer architecture is computationally expensive. Further, it is well known that the transformer architecture does not scale well to larger sequences. The self-attention mechanism imposes a compute complexity of $O(n^2)$ during training and $O(n)$ during inference, even after using the KV cache, with respect to input length $n$. Moreover, as the blocklength scales, a memory complexity of $O(n^2)$ prohibits training the algorithm from using a large batch size, which is crucial for attaining a good performance for any deep-learning models. 

An alternative approach would be to design a symbol-by-symbol coding scheme that can be scaled to any blocklength $L$ by encoding $K$ bits at a time independently. Within this context, an important question is: what is the extent of performance degradation compared to neural block coding schemes like GBAF? Moreover, it is necessary to formulate a novel and simplified architecture tailored to symbol-by-symbol processing. Finally, through streamlining the architecture and confining to symbol-by-symbol schemes, can we analyze and interpret the codes learned by deep learning models, discerning the reasons behind their notably superior performance compared to analytical counterparts?

In the coming sections, we answer all these questions. In \secref{sec:deepcode}, we systematically present \lightcode, a lightweight symbol-by-symbol neural coding scheme, which achieves state-of-the-art BLER performance~(\secref{sec:results}). Further, we analyze GBAF to study the efficacy of block coding by performing a systematic ablation study and also analyze \lightcode to identify the crucial components necessary for achieving ultra-low BLER in~\secref{sec:analysis}.


% In \secref{sec:deepcode}, we systematically present \lightcode, a lightweight neural coding scheme, which achieves reliability (Sec VII). GBAF analysis ... interpetation of lightcode in section VIII. not necessary attention 


% In this scenario, a natural question to ask is what the degradation in performance is with respect to neural block coding schemes such as GBAF. Further, a new architecture suited for symbol-by-symbol needs to be developed. Additionally, by simplifying the architecture and limiting to symbol-by-symbol schemes, can we analyze and interpret the codes learned by these deep learning models and understand why the performance is significantly better than their analytical counterparts. 

% 1. what architecture will be good? 

% 2. would it be as good as complicated block-level codes? or is block level coding necessary?



% %% This leads us to question the necessity of block coding in GBAF.

% Additionally, how do we reduce the complexity of the network in the absence of blockcoding? 

% 3. symbol-level thing: 
% Finally, can we provide some interpretation of the codes learned by these deep learning models and understand why the performance is significantly better than their analytical counterparts? 





%to answer all of these questions. %{\color{red}Hyeji TODO}








==> jsac/noisy.tex <==
% \section{Coding for Channels with Noisy Feedback}\label{sec:noisy}
% Finally, we now consider the case of channels with noisy feedback \textit{i.e.,} $\sigma_{fb}^2 > 0$. While the assumption of noiseless feedback is easier to study, most practical feedback channels suffer from noise even when the receiver sending the feedback operates at high power. Because of this limitation, both SK and \gn schemes do not perform well. To address this,~\cite{chance2011concatenated} introduces a linear feedback scheme that is implemented as an inner code to a concatenated code, which was found to be optimal within the linear family of codes~\cite{agrawal2011iteratively}. More recently,~\cite{mishra2023linear} proposed using dynamic programming to improve the performance, which turns out to be a generalized version of SK. However, despite these improvements, the linearity of these schemes severely limits the performance that can be achieved. 

% \begin{figure}[!htb]
%     \centering
%  	\includegraphics[width=0.6\linewidth]{figs/bler_3_9_noisy.eps}
%  	\captionsetup{font=small}
%  	\caption{Performance comparison of \lightcode with GBAF and other existing neural feedback codes for rate $\sfrac{3}{9}$ and noisy feedback with SNR = $20$ dB. \lightcode achieves BLER performance comparable to GBAF while utilizing only $\sfrac{1}{10}^{\text{th}}$ the number of parameters.}
%  	\label{fig:bler_3_9_noisy}
% \end{figure}

% Recalling the deep-learning-based schemes introduced in~\prettyref{sec:neural_codes}, one of the interesting properties of these codes is their robustness to noise in the feedback channel. By taking advantage of the general deep-learning-based schemes for noiseless feedback, it is straightforward to inject noise into the feedback channel during training to make the encoder-decoder robust. Hence, learning-based schemes can help design a practically realizable class of codes that can trained purely in a data-driven fashion and can provide gains under both noiseless and noisy feedback settings.

% For training \lightcode on noisy feedback channels, empirically, we found that selecting the input features as the previous encoder outputs $x_1$ and the cumulative noise $n_i + \Tilde{n}_i$ separately works better than directly passing the feedback $\Tilde{y_i}$ from previous rounds, which was the choice for noiseless feedback. Except for the change in input feature, the rest of the architecture and training details remain the same as the noiseless feedback setting. 



==> jsac/powerblast.tex <==
\section{Proposed analytical coding scheme: \pb}\label{sec:pb}
In this section, we propose \pb, a hybrid 2-phase scheme, to iteratively refine the LMMSE estimate of the PAM symbol at the receiver and shift to a discrete symbol scheme that takes advantage of the sparsity of the error in the estimate of the PAM index in the final round. Through theoretical analysis and empirical results, we demonstrate that the performance of \pb is better than both SK and GN in several regimes of interest. 

For a rate $\sfrac{K}{D}$ code, \pb begins by mapping $K$ bits of information to a $2^K$ PAM constellation and transmits the symbols on the forward AWGN channel. The receiver performs an LMMSE estimate and sends the estimate as feedback to the transmitter through the noiseless feedback channel. This continues for the first $D-1$ rounds. In the final round, \pb uses a discrete symbol strategy to send the error in the PAM index of the estimate. The complete algorithm is described in~\algref{alg:PB}. 
% .  {\color{red} Algorithm 17???}

\begin{algorithm}[hbt!]
\caption{\pb coding scheme}
\label{alg:PB}

\KwInput{Message symbol $\Theta$, number of rounds $D$, forward noise variance $\sigma_{ff}^2$ }

\vspace{5pt}
\textbf{Round 1:}\
\textbf{Tx:} 
Power normalization: $x_1 = \sqrt{P}\Theta$\;
Forward channel: $y_1 = x_1 + n_1$\;
\textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\Theta}_1 = \frac{\sqrt{P}y_1}{P + \sigma_{ff}^2};$ 

\vspace{5pt}
\texttt{/* Tx communicates the error in estimate $\hat{\Theta}_1 - \Theta$ over the next $D-2$ rounds */} \\
\vspace{5pt}

\While{$2 \leq i \leq D-1$}{
    \textbf{Tx:} Compute the error in estimate of previous round  ${\epsilon}_{i-1} = \hat{\Theta}_{i-1} - \Theta$ \;
    Power normalization: $x_i = \frac{\sqrt{P}}{\sigma_{i-1}} {\epsilon}_{i-1}$, $\sigma^2_{i-1} = \mathbb{E}[\epsilon^2_{i-1}]$\;
    Forward channel:  $y_{i} = x_{i} + n_{i}$\;
    \textbf{Rx:} LMMSE estimate of transmit symbol $\hat{\epsilon}_i = \frac{\sqrt{P}\sigma_{i-1}}{P + \sigma_{ff}^2} y_{i}$ \;
    \vspace{5pt}
    Update the estimate of $\Theta$ as: $\hat{\Theta}_i = \hat{\Theta}_{i-1} - \hat{\epsilon}_{i-1}$
}

\vspace{5pt}
\textbf{Decoding after round $D-1$}: Map $\hat{\Theta}_{D-1} = \frac{\hat{x_1}}{\sqrt{P_1}\eta}$ to the closest symbol in the $2^K$ PAM constellation.

\vspace{5pt}
\texttt{/* High-SNR scheme for final round */} \\
\vspace{5pt}

\textbf{Round D:}\
\textbf{Tx:} Compute the difference in PAM indices $U = \hat{M} - M$, where $\hat{M}$ and $M$ correspond to the integer index from PAM constellation for $\hat{\Theta}$ and $\Theta$ respectively\;
Power normalization: $x_D =  \frac{\sqrt{P}U}{\sigma_{ff}}$;
Transmit: $y_D = x_D + n_D$\; 
% \textbf{Rx:} Send feedback as LMMSE estimate of transmit symbol $\E [U_2 | y_2] = \frac{\sigma_2 \sqrt{P_2}y_2}{1 + P_2}$\;
% \vspace{5pt}
% Update the estimate as $\hat{x_1} = x_1 - \E [U_2 | y_2]$
\vspace{5pt}
\textbf{Final Decoding}: Use MAP decoder to detect $\hat{U}$ and detect original PAM signal using $\hat{U}$.


\end{algorithm}
% \vspace{-1em}

We note that \pb can be seen as a combination of SK and GN. Rate $\sfrac{K}{D}$ \pb can be interpreted as $D-1$ rounds of rate $\sfrac{K}{D}$ SK scheme with LMMSE estimate, followed by the discrete variant of GN scheme for the final round, resulting in a non-negligible improvement in performance in certain regions of SNR. The error analysis for the \pb scheme % under the assumption of MVUE estimate after round 1 
is provided below. %% As for the SK scheme, for ease of analysis, we assume that the MVUE estimate is used at the end of round 1. <- This is already in the proof of Theorem, so we can skip it here. 

% The key difference between the SK scheme and the initial rounds of the GN scheme lies in the choice of information transmitted in the second round. In SK, the difference between $\Theta$ and the LMMSE  estimate $\hat{\Theta}$ is transmitted, whereas in GN, the noise in the channel realization from round 1, $\mathbf{n_1}$, is transmitted. Hence, \pb can be interpreted as $D-1$ rounds of SK scheme with LMMSE estimate, followed by GN scheme for the final round, resulting in a non-negligible improvement in performance in certain regions of SNR. The error analysis for the \pb scheme is provided below. 

% We now propose a variation to the GN scheme by combining the SK scheme and the discrete-symbol scheme of GN to demonstrate a noticeable improvement in performance using a simple modification. We refer to this new scheme as \pb.


% {\color{red}In this section, we propose the powerblast algorithm and show that it is better than both Sk and GN.. 


% Algorithm: Description first. And then say by the way,  this can be seen as SK plus GN... }

% . {\color{red} trimming}








% \begin{theorem}[Error Analysis.]
% After $D$ rounds of communications ......  \begin{equation}
%     p_e = 2(1-p_{SK})Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{SK}}} \right) + p_{SK}Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{SK}}} \right),
% \end{equation}
% where \begin{equation}
%     p_{SK} = 2(1 - 2^{-K})Q\left(   \sqrt{ \frac{3S (1+S)^{D-2}}{2^{2K}-1}     }       \right).
% \end{equation}

% \end{theorem}

\begin{theorem}[Error Analysis]
The probability of error for rate $\sfrac{K}{D}$ \pb scheme is given by
\begin{equation}
    p_{PB} = 2(1-p_{SK})Q \left( \gamma \sqrt{S} \right) + p_{SK}Q \left( \left( \frac{1}{p_{SK}} - \gamma\right) \sqrt{S} \right)
\end{equation}
where \begin{equation}
    p_{SK} =  2(1 - 2^{-K})Q\left(   \sqrt{ \frac{3S(1+S)^{D-2}}{2^{2K}-1}     }       \right)
\end{equation}
and $\gamma$ denotes the detection threshold and $S$ denotes the SNR of the forward AWGN channel on a linear scale, and $Q()$ is the standard Q-function.%\textit{i.e.,} the tail distribution function of the standard normal distribution.
\end{theorem}

\begin{proof}
        % \subsection{Error Analysis}
        % We now analytically compute the probability of error for \pb scheme. 
        We begin by computing the probability of error for phase 1, which consists of $D-1$ rounds of the SK scheme. For ease of analysis, we follow the same assumption of ~\cite{ben2017interactive}, where the estimator after round one is assumed to be MVUE instead of LMMSE, implying,
        \begin{equation}
            \hat{\Theta}_1 = \frac{y_1}{\sqrt{P}}.
        \label{eq:mvue}
        \end{equation}
        Further, based on~\algref{alg:SK}
        % 
        , we can view the effective channel corresponding to rounds 1 to $D-1$ as one round with effective SNR $S.(1+S)^{D-2}$, $S = \sfrac{P}{\sigma_{ff}^2}$ is SNR for the forward channel in linear scale. It is straightforward to show that the probability of error incurred in transmitting a symbol from unit power normalized $2^K$ PAM, using an optimal detector, is
        \begin{align*}
            p_e &= 2(1 - 2^{-K})Q\left(\frac{\sqrt{P}\eta}{\sigma} \right)\\
                &=  2(1 - 2^{-K})Q\left(    \sqrt{ \frac{3S}{2^{2K}-1}     }     \right),
        \end{align*}
        where $S$ is the forward channel SNR in linear scale and $Q()$ is the Q-function. Hence, the effective probability of error after $D-1$ rounds of SK is
        \begin{equation}
            p_{SK} = 2(1 - 2^{-K})Q\left(   \sqrt{ \frac{3S(1+S)^{D-2}}{2^{2K}-1}     }       \right).
        \end{equation}
        
        We now proceed to compute the probability of error for phase two, which is transmitting the difference in integer (message) index over an AWGN channel. The key assumption for the high-SNR region is that the noise variance is small enough (compared to the effective forward SNR) that any errors beyond decoding to adjacent PAM symbols \textit{i.e.,} errors beyond 1 index difference are essentially negligible~\cite{gallager2009variations}. Hence, the problem can be rephrased as finding the probability of error to communicate a symbol from the constellation $\{ -1, 0, 1 \}$, with probability distribution $\{ \sfrac{p_{SK}}{2}, 1 - p_{SK}, \sfrac{p_{SK}}{2} \}$ using MAP decoder. This can be computed as
        \begin{equation}
            % p_{PB} = 2(1-p_{SK})Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{SK}}} \right) + p_{SK}Q \left( \frac{1}{2} \sqrt{\frac{S}{p_{SK}}} \right).
            p_{PB} = 2(1-p_{SK})Q \left( \gamma \sqrt{S} \right) + p_{SK}Q \left( \left( \frac{1}{p_{SK}} - \gamma\right) \sqrt{S} \right),
        \end{equation}
where $\gamma$ is the detection threshold and $S$ is the SNR of the forward AWGN channel on a linear scale.
         
\end{proof}

% \medskip

\noindent \textbf{\pb vs. SK and GN  schemes.} 
The key difference between \pb and SK is in the last round of communication, where \pb shifts to a discrete symbol scheme, as seen in line 13 of~\algref{alg:PB}, by taking advantage of the high effective SNR over the initial $D-1$ rounds \textit{i.e.,} the (effective) noise variance is much smaller than the distance between adjacent PAM symbols. Hence, it is beneficial to now transmit the error in the PAM constellation index, which lies in $\{-1, 0, 1\}$ with a very high probability, resulting in a much lower probability of decoding error.

Further, compared to GN, the key difference in \pb is the choice of information transmitted after round 1. GN communicates and refines the noise from round 1, $n_1$, starting round 2, as seen in line 4 of~\algref{alg:GN}. In contrast, \pb transmits and refines the error in LMMSE estimate of $\Theta$, as seen in line 4 of~\algref{alg:PB}. It is seen from~\cite{ben2017interactive} that the effective SNR (in linear scale) after $D$ rounds is given by $S(1+S)^{D-1}$ for GN and $(1+S)^{D} - 1$ for \pb. %and the effective SNR for \pb which uses LMMSE after round 1 is given by $(1+S)^{D} - 1$. 
% 
While the difference in effective SNR becomes negligible for large $D$, it can be significant when operating for a finite number of rounds, resulting in the superior performance of \pb.

% {\color{red} This needs to be revisited.}\textcolor{violet}{Updated; needs to be reviewed.} {\color{brown} lower case theta undefined}

The performance comparison between the error expressions for a general SNR and rate is not straightforward (as they are represented in terms of Q functions). Instead, we limit our comparison to the canonical settings considered in the recent literature on channels with feedback (e.g.,~\cite{ozfatura2022all}), for rates $\sfrac{3}{6}$ and $\sfrac{3}{9}$ and plot the BLER performance in~\figref{fig:bler_gn_vs_pb}; we observe %to demonstrate 
significant gains of \pb compared to both SK and GN in terms of the BLER performance. 




% \textcolor{blue}{ We attribute the impressive gains of \pb over SK and GN to the choice of estimator after round 1. To simplify the error analysis, the estimator after round 1 in SK uses MVUE estimate of the transmitted symbol $\hat{\Theta}_1$, as seen in line 3 of ~\algref{alg:SK}~\cite{ben2017interactive} and also in~\eqref{eq:mvue}. This assumption is necessary in showing an exponentially decaying error exponent for SK but is not optimal for minimizing the decoding error after finite rounds of communication. It is seen from~\cite{ben2017interactive} that the effective SNR (in linear scale) after $D$ rounds is given by $S(1+S)^{D-1}$ using an MVUE estimate whereas $(1+S)^{D} - 1$ when using LMMSE estimate, where $S$ is the SNR in linear scale for forward AWGN channel. While the effective SNR converges to the same value for the asymptotic case of $D \to \infty$, the difference in effective SNR becomes significant for finite rounds of communication. Further, instead of refining the error in estimate, GN aims to communicate the noise realization from round 1~\cite{gallager2009variations}, as shown in line 4 of~\algref{alg:GN}, which is the strategy developed by Elias~\cite{Elias1956ChannelCapacity} to communicate a Gaussian random variable. While this a suitable strategy for achieving an exponentially decaying error exponent, this also does not optimize for the BLER performance after finite rounds of communication, as seen in~\figref{fig:bler_gn_vs_pb}. Hence, by using the LMMSE estimate and iteratively refinig the error in estimate, \pb achieves a superior performance for a given finite number of rounds of communication. }


% , SK uses a MVUE after round 1~\cite{ben2017interactive}, as seen in Alg. 2 line 3 and communicates the noise $Z_0$ from round 1 over the remaining $D-1$ rounds~\cite{gallager2009variations}. Similarly, GN sends $Z_0$ as feedback after round 1 and follows the same strategy, as shown in line 4 of Alg. 4. From~\cite{ben2017interactive}, it is seen that the effective SNR after $D$ rounds is given by $S(1+S)^{D-1}$ using an MVUE estimate whereas $(1+S)^{D} - 1$ when using LMMSE estimate. While the effective SNR converges to the same value for the asymptotic case of $N \to \infty$, for finite rounds of communication, the difference in effective SNR becomes significant. Hence, by using the LMMSE estimate and transmitting the error in estimate, \pb achieves a superior performance for a given finite number of rounds of communication. 
% {\color{red} This needs to be revisited. Algorithm 2 is for PowerBlast. Also instead of just saying that SK uses a MVUE, say `uses a MVUE to do what' -- like estimate the noise $Z_0$ also D vs N}


% From Alg. 2 line 3, we observe that SK uses an minimum-variance unbiased estimator (MVUE) estimator~\cite{schalkwijk1966coding_p1,ben2017interactive}. In order to make the error analysis tractable, this is a valid assumption, and does not make a difference in asymptotic region. As a result, the SK scheme achieves an exponentially decaying error. On similar lines, GN transmits the noise $Z_0$ starting from round 2~\cite{gallager2009variations}, as shown in line 4 of Alg. 4. When operating in non-asymptotic regime, the choice of estimator after round 1 makes a significant difference in effective SNR across the rounds of communications. From~\cite{ben2017interactive}, it is seen that the effective SNR after $D$ rounds is given by $S(1+S)^{D-1}$ using an unbiased estimator whereas $(1+S)^{D} - 1$ when using LMMSE estimator. While the effective SNR converges to the same value for the asymptotic case of $N \to \infty$, for finite rounds of communication, the difference in effective SNR becomes significant. Hence, by using the LMMSE estimate and transmitting the error, instead of using unbiased estimate and transmitting the noise, \pb achieves a much superior performance for a given finite number of rounds of communication. 



% \textcolor{blue}{One major reason for this superior performance is the choice of estimator at the receiver after round 1. While \pb focuses on the BLER performance for a given number of rounds of communication in the finite regime, both SK and GN schemes focus on performance in the asymptotic region, to demonstrate an exponentially decaying error expression. In order to make this analysis tractable, both schemes assume an unbiased estimator after round 1~\cite{ben2017interactive} and transmits the noise $Z_0$ using the remaining $D-1$ rounds~\cite{gallager2009variations}. While this assumption is valid and does not make a difference for the asymptotic case of $N \to \infty$, for finite rounds of communication, the difference in effective SNR becomes significant. Hence, by using the LMMSE estimate and transmitting the error, instead of using unbiased estimate and transmitting the noise, \pb achieves a much superior performance for a given finite number of rounds of communication. }


% {\color{red} Generally can we say one is always better than the other(s)? if not, we admit that fact, and then say for some settings -- the common benchmark in recent work -- PB is better than SK, which is better than GN. }
% %SK vs. GN vs. PowerBlast: 
% In \figref{fig:bler_gn_vs_pb}, we compare the BLER performance, demonstrating significant gains for rates $\sfrac{3}{6}$ and $\sfrac{3}{9}$ \pb scheme, outperforming both SK and GN. 
% The gain is substantial.} 

% \begin{figure}[ht]
% \centering 
% \begin{minipage}[b]{0.45\linewidth}
%   \centering
%   \subfloat[Rate $R = \sfrac{3}{6}$]{%
%     \includegraphics[clip,width=\linewidth]{figs/bler_gn_vs_pb_3_6.pdf}
%   }
% \end{minipage}
% \hspace{0.05\linewidth} % Adjust the horizontal space between the figures
% \begin{minipage}[b]{0.45\linewidth}
%   \centering
%   \subfloat[Rate $R = \sfrac{3}{9}$]{%
%     \includegraphics[clip,width=\linewidth]{figs/bler_gn_vs_pb_3_9.pdf}
%   }
% \end{minipage}
% \captionsetup{font=small}
% \caption{By combining SK and discrete-symbol strategy of GN scheme, \pb noticeably improves the BLER performance upon both SK and GN schemes.}
% \label{fig:bler_gn_vs_pb}
% \end{figure}

\begin{figure}[ht]
\centering 
\begin{minipage}[b]{0.9\linewidth}
  \centering
  \subfloat[Rate $R = \sfrac{3}{6}$]{%
    \includegraphics[clip,width=\linewidth]{figs/bler_gn_vs_pb_3_6.pdf}
  }
\end{minipage}
\vspace{0.5cm} % Adjust the vertical space between the figures
\begin{minipage}[b]{0.9\linewidth}
  \centering
  \subfloat[Rate $R = \sfrac{3}{9}$]{%
    \includegraphics[clip,width=\linewidth]{figs/bler_gn_vs_pb_3_9.pdf}
  }
\end{minipage}
\captionsetup{font=small}
\caption{By combining the SK and discrete-symbol strategy of the GN scheme, \pb noticeably improves the BLER performance upon both SK and GN schemes.}
\label{fig:bler_gn_vs_pb}
\end{figure}



%\end{remark}



% {\color{red} Qn: How do we talk about the performance comparison with GBAF here?} Ans: not in detail, but a slight hint to what is coming next will be a good addition.

% {\color{blue} Transition: In the next section, we consider deep learning based ones... PowerBlast will serve as a solid analytical baseline. Surprisingly we will see that PB is sometimes comparable...... but not always... }

From the results so far, we have demonstrated that \pb provides the best performance among the analytically tractable solutions for channels with noiseless feedback that are recently considered in the literature (to demonstrate the reliability of deep-learning-based coding schemes~\cite{ozfatura2022all}). In the coming sections, we consider deep-learning-based coding schemes such as GBAF and show that, surprisingly, the analytical \pb coding scheme often delivers %while analytical solutions deliver 
competing performance. Nevertheless, \pb still falls short when the SNR is very low; thus, we investigate conditions under which deep-learning-based schemes provide the highest gain. Finally, we propose \lightcode, a lightweight neural coding scheme that achieves state-of-the-art performance with very low complexity.

% that can provide performance that can compete with deep learning based solutions in some scenarios. For instancz, 

% followed by a high-SNR variant in the final round.



% It is clear that deep learning based channel codes are extremely reliable but also come with a huge computational cost. Hence it is crucial to investigate the merit of such schemes carefully and compare the performance with classical feedback coding schemes.

% In this work, we look at block length $K=3$ and compare the performance of deep learning based schemes against SK and 2-phase \gn schemes. Additionally, we propose a new scheme based on the combination of SK and 2-phase \gn scheme that can provide noticeable improvements in performance using simple modifications. We refer to this scheme as \pb.





% Through extensive empirical and theoretical analysis, we observe that neural feedback codes are the most useful in regions of very low SNR with respect to the rate of communication and in regions of high-SNR, simple schemes are sufficient to achieve extremely low BLER. To demonstrate this, we present the comparison of GBAF with \pb in \prettyref{fig:classical}for two rates $\sfrac{3}{9}$ and $\sfrac{3}{6}$. 

% \begin{figure*}[!htbp]

% \centerline{
% % \hspace{-0.1in}
% \subfigure[]
% {
%     \centering
%  	\includegraphics[width=0.5\linewidth]{figs/bler_pb_3_6_noiseless.pdf}
%     % \caption{Rate $\sfrac{3}{6}$}
%  	\label{fig:bler_pb_3_6}
% }
% \hspace{-0.25in}
% \subfigure[]
% {
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/bler_pb_3_9_noiseless.pdf}
%  	\label{fig:bler_pb_3_9}
%   }

%  \vspace{-0.5em}
%   }
%   \captionsetup{font=small}
%   \caption{Performance comparison of GBAF~\cite{ozfatura2022all} with 2-phase \gn \cite{gallager2009variations} and \pb (ours) for noiseless feedback. BLER results show that \pb is significantly better than 2-phase \gn for (a) rate-$\sfrac{3}{6}$ and (b) rate-$\sfrac{3}{9}$. Additionally, it is clear that given a sufficiently high-SNR, classical feedback coding schemes can be as good as or better than deep learning based feedback coding schemes. Note that we mark BLER $\approx 0$ as $10^{-11}$ to make the visualization easy.}
% \vspace{-1.5em}
% \end{figure*}\label{fig:classical}

==> jsac/related_works.tex <==
\section{Related Works}\label{sec:rel_works}
In this section, we briefly review the current state of coding for channels with passive feedback. Existing feedback communication schemes can be broadly classified into two categories. The first is human-crafted codes that are carefully designed to improve the error correction probability after each round in a sequential manner. The seminal work of Schalkwijk-Kailath \cite{schalkwijk1966coding_p1,schalkwijk1966coding_p2} used a fixed block length coding scheme with $2^K$-ary PAM constellation, $K$ is block length. It demonstrated that feedback could result in a second-order exponential decay of decoding error for all transmission rates less than capacity. Later, Zigangirov \cite{zigangirov1970upper} demonstrated that for the case of finite bandwidth, the doubly exponential bound can be replaced by $K^{\th}$ order exponential bounds for asymptotically large lengths. Similar lines of work can be found in \cite{martins2008coding,gallager2009variations,chance2011concatenated,kim2007gaussian,ben2017interactive}. While these schemes promise impressive theoretical guarantees in terms of performance, they quickly suffer from numerical precision issues in practice, as the length increases. Hence, commonly used schemes in practice are still limited to ARQ and HARQ, which do not fully utilize the capabilities of the available high-fidelity noiseless feedback channel, as demonstrated by CE-HARQ\cite{ankireddy2023compressed}.

% Commonly used schemes in practice are Automatic Repeat Request (ARQ) and Hybrid Automatic Repeat Request (HARQ), which utilize simple 1-bit feedback from the receiver to indicate success by acknowledgment (ACK) or a failure by negative acknowledgment (NACK). These schemes are primitive and do not  


Recent advances in machine learning and deep learning enabled the creation of a new line of work in the area of channel coding by leveraging the expressive power~\cite{raghu2017expressive} of deep neural networks. Several works explored various approaches to improving the performance of channel codes for point-to-point channels ranging from augmenting classical decoder with learnable parameters~\cite{nachmani2016learning, nachmani2018deep, ankireddy2023interpreting, hebbar2022tinyturbo} to creating novel neural network architectures based neural encoders and decoders~\cite{hebbar2023crisp, hebbar2024deeppolar} and improving the code design using sequential models~\cite{li2021learning,ankireddy2024nested}. Another line of work explored coding for channels with feedback, where deep learning techniques were used to design new encoding and decoding schemes by taking advantage of the high-capacity feedback channel. In this aspect, the seminal work by Kim et al. Deepcode~\cite{kim2018deepcode} modeled both encoder and decoder functions as recurrent neural networks (RNNs) to process a bit stream in a sequential manner to directly minimize the end-to-end transmission error over an AWGN channel. This was further extended in deep extended feedback (DEF) codes~\cite{safavi2021deep} to introduce modulation to increase spectral efficiency and also to use more power sequential models such as long short-term memory (LSTM) architecture to model the dependency over higher rounds of communication. Further, in~\cite{mashhadi2021drf}, deep SNR-robust feedback (DRF) codes were introduced, which explored the generalization of Deepcode and DEF codes to multiple SNRs using SNR-aware attention and curriculum training with batch size scheduling. Later, a new level of performance was achieved by replacing RNNs and LSTM models with self-attention based transformer models in AttentionCode~\cite{shao2023attentioncode}. More recently, generalized block attention feedback (GBAF) codes were introduced in~\cite{ozfatura2022all}, which is currently the state-of-the-art deep learning-based feedback code with passive feedback. GBAF uses a self-attention mechanism to do block coding across the codeword, introducing dependencies across the positions and improving the decoding performance by an order of magnitude over the previous deep learning-based feedback codes. This clearly demonstrates that a new level of error-correcting performance for feedback codes can be achieved by leveraging advances in deep learning. In another work, Robust Coding~\cite{kim2023robust} focused on designing codes for channels with noisy feedback using bi-directional attention-based decoding architecture. But these state-of-the-art solutions come at an increasingly high computational cost, potentially exponentially more complex compared to human-crafted codes, and motivate us to look for low-complex solutions. We also note that further improvements can be achieved by using active feedback~\cite{chahine2022inventing,ozfatura2022feedback}, but we limit ourselves to passive feedback in this work. 

==> jsac/results.tex <==
% \section{Results on Channels with noiseless/noisy feedback}\label{sec:results}

\section{Main Results }\label{sec:results}

We begin by comparing the performance of \lightcode with the current state-of-the-art in deep-learning-based coding schemes for noiseless passive feedback setting, GBAF~\cite{ozfatura2022all} and other schemes, demonstrated in~\figref{fig:bler_3_9_noiseless}. Next, we discuss a method for extending \lightcode to moderate block-length regimes of up to $L=51$ and study the performance.  

Finally, we look at deep-learning-based coding schemes for noisy feedback settings and how \lightcode can be extended to this setting with minimal changes. We then proceed to compare the BLER performance for the same configuration as before but with a feedback SNR of $20$ dB. 



%{\color{blue} We do two things: First, compare \lightcode and PowerBLAST against existing neural codes on the representative setup (fig 5) and various rates. Next, consider extending the blocklength.  One option is to talk about results on noisy feedback here as well - subsection (c). Pros: Results section will be longer. We have quite a lot of sections at the moment, reducing one can be good. Cons: a slight de-emphasis on noisy feedback.} {\color{red} Updated}

\subsection{\lightcode and \pb vs. existing neural codes for noiseless feedback}\label{sec:comparison}



In this section, we evaluate the performance of \lightcode and \pb and compare them against several existing analytical and deep-learning feedback schemes. For concreteness, we consider the canonical setting of rate $R=\sfrac{3}{9}$ with block length $K=3$ and $D=9$ rounds of communication on AWGN forward channel and noiseless feedback.

% and compare against several existing deep learning-based feedback codes. 

\medskip

\textbf{Baselines.} Our primary comparison is against GBAF~\cite{ozfatura2022all}, which is the current state-of-the-art for the noiseless passive feedback setting. Additionally, we consider Deepcode~\cite{kim2018deepcode}, DEFC~\cite{safavi2021deep}, DRFC~\cite{mashhadi2021drf}, Attentioncode~\cite{shao2023attentioncode}, and Robust Coding~\cite{kim2018deepcode}. Further, for completeness as well as to understand the relative gains of deep-learning-based coding schemes, we also compare the performance against NR-LDPC~\cite{Huawei2017LDPC}, Schalkwijk-Kailath~\cite{schalkwijk1966coding_p1}, \gn~\cite{gallager2009variations} and \pb. 

\textbf{Results.} In~\figref{fig:bler_3_9_noiseless}, we compare the BLER performance of rate $\sfrac{3}{9}$ coding schemes. We train a pair of encoder-decoder models at each SNR point in the plot.
% for a noiseless passive feedback channel. 
\lightcode consistently outperforms the existing deep-learning-based schemes, including GBAF, while utilizing $< \sfrac{1}{10}^{\text{th}}$ the number of parameters. Interestingly, these results indicate that \pb surpasses the performance of all existing schemes, including \lightcode, when an adequately high signal-to-noise ratio is provided, which is $-0.5$ dB for rate $\sfrac{3}{9}$. However, the performance of deep-learning codes is significantly better at lower SNRs. Here, we highlight that by utilizing the clean feedback, \lightcode and \pb achieve an extremely small error rate even when operating at $0.75$ dB below the channel capacity. Further, we note that because of the extremely short block lengths considered, it is hard to derive meaningful achievability or converse bounds, such as~\cite{polyanskiy2010channel}, where blocks lengths of $100$ or higher are considered.

The blocklengths considered for the baselines in~\figref{fig:bler_3_9_noiseless} are listed in~\tabref{tab:block_lengths}, where $K=50$ for some of the schemes, which is larger than the length $K=3$ considered for rest of the schemes including \lightcode. While the BLER comparison against the different blocklengths is unfair, to maintain consistency, we used the same methodology followed in the current state-of-the-art results, including GBAF~\cite{ozfatura2022all} and Robust Coding~\cite{kim2023robust}. For a fairer comparison, we propose a modular approach for extending \lightcode to larger blocklengths in~\secref{sec:long_length}.


\begin{table}[!ht]
\centering
\begin{tabular}{lc}
\hline
\textbf{Scheme} & \textbf{Message length $K$} \\
\hline
%NR-LDPC & $\approx 51$ \footnotemark[1] \\
Deepcode & $50$ \\
DEFC & $50$ \\
DRFC & $50$ \\
AttentionCode & $50$ \\
\gn & $3$ \\
\pb & $3$ \\
Robust Coding & $3$ \\
GBAF & $3$\footnotemark[1] \\
\lightcode & $3$ \\    
\hline
\end{tabular}
\captionsetup{font=small}
\caption{Block lengths of different coding schemes.}
\label{tab:block_lengths}
\end{table}

%\footnotetext[2]{As indicated in~\cite{ozfatura2022all}. We thank the authors for providing the raw data for plotting the baselines.}

\footnotetext[1]2{While GBAF uses a blocklength of $51$, the BLER in~\cite{ozfatura2022all} was reported for the sub-block of length $3$.}



% {\color{red} I still find it weird talking about the blocklength only in Subsection B. As you present Figure 6, you should talk about the basic setup and stuff. Move the first paragraph in B and Table VI to this section. } \textcolor{violet}{Moved the discussion of difference in blocklengths to Results. mentioned that we will talk about extending \lightcode to longer blocklengths in section B.}

\begin{figure}[!htb]
    \centering
 	\includegraphics[width=\linewidth]{figs/bler_3_9_noiseless_jsac.pdf}
 	\captionsetup{font=small}
 	\caption{Noiseless feedback: Performance comparison against existing classical and neural feedback codes for rate $\sfrac{3}{9}$. \pb achieves the best performance among existing classical schemes and performs comparable to state-of-the-art neural coding schemes in high-SNR regions. \lightcode achieves superior BLER performance compared to GBAF while utilizing $< \sfrac{1}{10}^{\text{th}}$ the number of parameters.}
 	\label{fig:bler_3_9_noiseless}
% \vspace{-1em}
\end{figure}


% \medskip 

\textbf{Multiple rates.} The coding rate of \lightcode is determined by two factors, block length $K$ and number of rounds of communication $D$. We keep the block length constant and vary $D$ to compare the performance against GBAF across multiple rates, as shown in~\tabref{tab:multi_rate}. \lightcode consistently outperforms GBAF across a range of rates $\{ \sfrac{3}{9}, \sfrac{3}{8}, \sfrac{3}{7}, \sfrac{3}{6}, \sfrac{3}{5}\}$, while utilizing a fraction of the number of parameters. 

% reference from GBAF JSAIT paper 
\begin{table}[!htp]
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{SNR (dB)} & \textbf{Rate} & \textbf{GBAF} & \textbf{\pb} & \textbf{\lightcode} \\
\midrule
$-1.0$ & $3/9$ & $7\times 10^{-10}$ & $2.8\times 10^{-4}$ & $\mathbf{4.5\times 10^{-10}}$ \\
$0.0$ & $3/8$ & $6.1\times 10^{-8}$ & $8.8\times 10^{-7}$ & $\mathbf{5.1\times 10^{-9}}$ \\
$1.0$ & $3/7$ & $7.5\times 10^{-8}$ & $1.0\times 10^{-8}$ & $\mathbf{1.0\times 10^{-8}}$ \\
$2.0$ & $3/6$ & $1.5\times 10^{-6}$ & $1.5\times 10^{-8}$ & $\mathbf{8.3\times 10^{-7}}$ \\
$3.0$ & $3/5$ & $8.7\times 10^{-7}$ & $1.9\times 10^{-4}$ & $\mathbf{2.7\times 10^{-7}}$ \\
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{BLER performance comparison of \lightcode with GBAF with \pb for different rates. \lightcode consistently performs better than GBAF while using $< \sfrac{1}{10}^{\text{th}}$ the number of parameters.}
\label{tab:multi_rate}
\vspace{-1em}
\end{table}

% \medskip

\textbf{Error floor.} As observed in~\figref{fig:bler_3_9_noiseless}, \lightcode exhibits an error floor in the high-SNR region, similar to the existing deep-learning-based coding schemes such as Deepcode and GBAF. We believe a key reason for this behavior is the difficulty of training the decoder in the high SNR region, where the error events are extremely rare. For instance, while training in the regime of BLER $10^{-9}$, most of the training batches (batch size $10^5$) are error-free and do not provide sufficient guidance for the gradient descent to learn useful information, leading to saturation in performance.

% Specialized training techniques could be employed to address this issue, as demonstrated recently in~\cite{kwak2023boosting}.} 

% {\color{red} We should relate this paragraph to our results. Sure, we can talk about all existing learning-based schemes, but what matters more is the schemes that we consider -- do you wanna say LIGHTCODE as well as learning-based schemes such as Deepcode, DEFC, blah blah? It's not just the existing learning-driven schemes. LIGHTCODE also has error floor.}


% Two major factors can be attributed towards this limitation. The first is the difficulty of training the model is high SNR region where the probability of block error is less than $10^{-9}$ and most of the training batches being error free. Since the total number of error events during training phase is negligible compared to the error-free events, the gradient descent is not very efficient, resulting in a potential saturation of the encoder-decoder. Additionally, reliably simulating the inference in high-SNR region is also challenging for the same reason. For all the simulation results presented in this work, we consider at least 100 block error events to guarantee the reliability of the results to a certain degree and the high-SNR results in GBAF considers 20 error events, limited by the time taken for simulation.  

% {\color{red}Two factors - one is the training aspect, and the other is measuring the BER? Is the latter a reason for the error floor?}



\subsection{Performance in moderate blocklength regime}\label{sec:long_length}

% {\color{blue}\textbf{Comparing different schemes:} 


 We now present a modular way to scale \lightcode to larger block lengths to enable a fair comparison against baselines with longer blocklengths. As a result of the curse of dimensionality, it is well known that the hardness of learning a code increases considerably with an increase in block length. As seen from results in Appendix~\secref{app:long_lightcode}, directly increasing the blocklength for \lightcode results in a poor BLER performance.
GBAF~\cite{ozfatura2022all} uses a computationally intensive transformer for performing block coding to support a length of $51$. To keep the complexity low, \lightcode instead uses a short blocklength $K$ (e.g., $K=3$) and treats a block of $L$ bits as $l = \sfrac{L}{K}$ independent sub-blocks. This modular approach of encoding $K$ bits at a time is motivated by ablation studies that demonstrate the negligible benefit of block coding in GBAF, presented in detail in~\secref{sec:ablation}. Thus, the resulting BLER for a blocklength $L$ \lightcode can be computed as
% {\color{red}Here we're throwing this equation without providing the background on why we consider this or what we're planning to do. We should begin this section by stating what we do (eg VARY the length L and compare Lightcode against the baselines (fairly)) -- the BLER equation should come after that. Now I am curious why did we remove L=200 or 300?}
\begin{equation}
    p_L = 1 - (1-p_K)^l,
\label{eq:bler_modulo}
\end{equation}
where $p_L$ is the BLER for blocklength $L$ and $p_K$ is the BLER for blocklength $K$.

Finally, for a fair comparison against schemes with block length $K=50$, we refer to the results in~\figref{fig:bler_3_9_noiseless_51} where we compute the BLER for blocklength $L=51$ for \lightcode using the modular approach presented above. At a forward SNR of $-1.0$ dB, \lightcode with blocklength $51$ has a BLER of $7 \times 10^{-9}$ which is significantly smaller than Deepcode, DEFC, DRFC, and AttentionCode that use a block length of $50$, demonstrating the superior performance of \lightcode even at moderately longer blocklengths. We note that the BLER $p_L$ approaches $1$ for very large values of $L$, but we restrict our study to the relatively short block length regime of $L<300$, where the performance is still superior to the baselines as demonstrated in~\figref{fig:bler_3_9_noiseless_51}. Further potential performance improvements at longer blocklengths may be achievable through a concatenated coding scheme that employs an outer block code, as explored in~\cite{chance2011concatenated}; we leave this as a direction for future work. %Further, performance improvements at longer blocklengths can also by utilizing an outer blocking coding scheme, as studied in~\cite{chance2011concatenated}, which we leave for future work.   
% \textcolor{red}{Chance-Love paper. as a future work}

% while maintaining the same architecture and complexity for encoder-decoder.} 



% \textcolor{red}{Updated the entire section; needs to be reviewed.}

% in~\secref{sec:ablation}, which demonstrate that explicit block coding is not beneficial in this regime and does not scale well. 

% Second is the increase in computational complexity of both encoder and decoder modules associated with block coding.  Results from~\figref{fig:bler_3_9_noiseless_51} illustrate that \lightcode scales gracefully with blocklength by independently encoding information in sets of $K=3$, keeping the complexity constant. Further, we also note that the bit error rate (BER) remains constant regardless of the blocklength $L$.

% Hence, instead of learning a longer blocklength, we propose keeping the blocklength short and treating a large block of information bits as sub-blocks of smaller blocklengths. For comparison, GBAF~\cite{ozfatura2022all} uses a self-attention based transformer to scale the block coding to length $51$. However, \lightcode achieves BLER superior to GBAF while using a code of length $3$ and treating a block of $51$ bits as $17$ independent sub-blocks of length $3$. {\color{brown}How does this paragraph fit into this subsection? performance in moderate blocklength regime?}


% {\color{brown} Where are you discussing the blocklengths for schemes in Figures 6,7,8? I see that it comes later. We're referring to Figure 6 many times. First is in the left column/page 10. Why not mention the blocklengths here? This section overall seems to be all over/unorganized. Take a look at the organization and try to merge old/new stuffs as appropriate.}
% Using a code designed for length $K$, it is straightforward to compute the probability of error for a larger blocklength $L$ by treating the message as a packet of $l = \sfrac{L}{K}$ independent sub-blocks. The packet error rate (PER) for a packet of size $l$ can be considered BLER for blocklength $L$, given by
% \begin{equation}
%     p_L = 1 - (1-p_K)^l,
% \label{eq:bler_modulo}
% \end{equation}
% where $p_L$ is the BLER for blocklength $L$ and $p_K$ is the BLER for blocklength $K$.

% This modular approach to encoding is motivated by two key observations. The first is from the ablation studies in~\secref{sec:ablation}, which demonstrate that explicit block coding is not beneficial in this regime and does not scale well. Second is the increase in computational complexity of both encoder and decoder modules associated with block coding.  Results from~\figref{fig:bler_3_9_noiseless_51} illustrate that \lightcode scales gracefully with blocklength by independently encoding information in sets of $K=3$, keeping the complexity constant. Further, we also note that the bit error rate (BER) remains constant regardless of the blocklength $L$.

\begin{figure}[t]
    \centering
 	\includegraphics[width=\linewidth]{figs/bler_3_9_noiseless_300_v3.pdf}
 	\captionsetup{font=small}
 	\caption{By independently encoding sub-blocks of length $K=3$, \lightcode provides a flexible way to encode for any blocklength $L$, providing a steady trade-off in BLER performance vs blocklength. Even at a block length of $50$, \lightcode significantly outperforms all baseline methods shown in~\figref{fig:bler_3_9_noiseless},  which utilize a maximum block length of $51$.}%\looseness=-1
  % without an increase in computational complexity.}} 
  % {\color{red} Can you also highlight the captions for figures that are updated? Minor issue, but I'm just thinking it'd be good to have more highlighted parts.}}
 	
% \vspace{-1em}
\label{fig:bler_3_9_noiseless_51}
\end{figure}




 % \textcolor{blue}{For a fair comparison against schemes with block length $K=50$, we refer to the results in~\figref{fig:bler_3_9_noiseless_51} where we compute the BLER for longer block length by treating a block of $L=51$ bits as $17$ sub-blocks, independently encoding $K=3$ bits into one symbol. Using~\eqref{eq:bler_modulo}, the BLER for blocklength $51$ can be computed as
 % \begin{equation}
 %     p_{51} = 1 - (1-p_3)^{17},
 % \end{equation}
 % where $p_3$ is the BLER of length $K=3$ scheme. Hence BLER of length $51$ is higher than BLER of length $3$. But from~\figref{fig:bler_3_9_noiseless_51}, we can see that this is still significantly smaller than the baselines with blocklength $50$, demonstrating the superior performance of \lightcode even at moderately longer blocklengths.}

\subsection{Coding for Channels with Noisy Feedback}\label{sec:noisy}
Finally, we now consider the case of channels with noisy feedback \textit{i.e.,} $\sigma_{fb}^2 > 0$. While the assumption of noiseless feedback is easier to study, most practical feedback channels suffer from noise even when the receiver sending the feedback operates at high power. Because of this limitation, neither the SK nor GN schemes perform well. To address this,~\cite{chance2011concatenated} introduces a linear feedback scheme that is implemented as an inner code to a concatenated code, which was found to be asymptotically optimal within the linear family of codes under AWGN forward channel~\cite{agrawal2011iteratively}. More recently,~\cite{mishra2023linear} proposed using dynamic programming to improve the performance, which turns out to be a generalized version of SK. However, despite these improvements, the linearity of these schemes severely limits the performance that can be achieved. 



Recalling the architecture of deep-learning-based schemes introduced in~\secref{sec:neural_codes}, one of the interesting properties of these codes is their robustness to noise in the feedback channel. By taking advantage of the general architecture, injecting noise into the feedback channel during training is straightforward to make the encoder-decoder robust. Hence, learning-based schemes can help design a practically realizable class of codes that can be trained in a data-driven fashion and can provide gains in noiseless and noisy feedback settings.

\begin{figure}[t]
    \centering
 	\includegraphics[width=\linewidth]{figs/bler_3_9_noisy_jsac.pdf}
 	\captionsetup{font=small}
 	\caption{\textcolor{black}{Noisy feedback: Performance comparison against existing neural feedback codes for rate $\sfrac{3}{9}$ and feedback SNR = $20$ dB. \lightcode achieves BLER performance comparable to GBAF while utilizing only $\sfrac{1}{10}^{\text{th}}$ the number of parameters.}}
 	\label{fig:bler_3_9_noisy}
% \vspace{-1em}
\end{figure}

For training \lightcode on noisy feedback channels, empirically, we found that selecting the input features as the previous encoder outputs $x_1$ and the cumulative noise $n_i + \Tilde{n}_i$ separately works better than directly passing the feedback $\Tilde{y_i}$ from previous rounds, which was the choice for noiseless feedback. Except for the change in input feature, the rest of the architecture and training details remain the same as the noiseless feedback setting. In~\figref{fig:bler_3_9_noisy}, we compare the performance of rate $\sfrac{3}{9}$ \lightcode against existing schemes, for a feedback SNR of $20$ dB. We see that \lightcode exhibits similar performance compared to GBAF while still utilizing only a fraction of the number of parameters. 

%% Main results : 2 directions

% 1: Showing the advantage of Sparse Code over SK + Gallager -- evident at higher lengths, can show results for length 51
% 2: Showing the advantage of Sparse Code over GBAF -- will be using length 17 results, 

% 





%% *** Two Result Figures ***

% Table: vs. AttentionCode 
% Figure: vs. AttentionCode (Rate 3/9) 

%% Comparison: Gallager vs. ListPowerBlast vs. Neural 

%% **** Interpretation ***


%% What is SparseCode learning?  %% Q1. (Concrete) are we perturbing %
%% - power scaling vs. direction/angles? 
%% Q2. (Abstract) Separate source-channel coding? 

%% *** Ablation studies *** 
% SparseCode/PowerBlast vs. Sparsity level 
% SparseCode/PowerBlast vs. SNR 

%% *** Complexity comparison *** 

% vs. AttentionCode for example. 





% \begin{figure}[!htb]
%     \centering
%  	\includegraphics[width=1.0\linewidth]{figs/bler_perf_temp.png}
%  	\captionsetup{font=small}
%  	\caption{BLER }
%  	\label{fig:bler}
% \end{figure}


% We compare the Block Error Rate (BLER) performance of SFC with SOTA DL-based block feedback code \cite{ozfatura2022all}. 



% - Figure: SNR vs BLER (Rate 1/3 ours vs. GBAF) 

% % % reference from GBAF JSAIT paper 
% % \begin{table}[!htp]\centering
% % \caption{Performance comparison}\label{tab: }
% % \scriptsize
% % \begin{tabular}{lrrrrrr}\toprule
% % \textbf{SNR (dB)} &\textbf{Rate} &\textbf{GBAF (nx7e4)} &\textbf{PB} &\textbf{SFC}  &\textbf{FC (100x7e4) } &\textbf{FC (7e4) }\\\midrule
% % -1 &3/9 &1.0e-9 &2.8e-4 &1.4e-4 &2.8e-6 &2.73e-6 \\
% % 0 &3/8 &6.1e-8 &8.8e-7 &2.5e-7  &1.12e-8 &1.34e-8 \\
% % 1 &3/7 &7.5e-8 &1.02e-8 &1.0e-8 &1e-8 &1.3e-8 \\
% % 2 &3/6 &1.5e-6 &3.25e-7 &9.3e-8 &2.5e-8 &1.45e-8 \\
% % 3 &3/5 &8.7e-7 &1.9e-4 &3.0e-5 &1.05e-6 &5.1e-7 \\
% % \bottomrule
% % \end{tabular}
% % \end{table}

% \begin{table}[!htp]\centering
% \caption{Performance comparison}\label{tab: }
% \scriptsize
% \begin{tabular}{lrrrrr}\toprule
% \textbf{SNR (dB)} &\textbf{Rate} &\textbf{GBAF (nx7e4)} &\textbf{FC (7e4)} &\textbf{PB} \\\midrule
% -1 &3/9 &1.0\times 10^{-9} &2.1e-6 &5e-4 \\
% 0 &3/8 &6.1e-8 &3.9e-9 &4.78e-7 \\
% 1 &3/7 &7.5e-8 &3.25e-9 &2.1e-9 \\
% 2 &3/6 &1.5e-6 &2.8e-9 &8.9e-8 \\
% 3 &3/5 &8.7e-7 &1.73e-7 &1.3e-4 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Fixed rate - higher-SNR: more gains 

% - Gallager: mega symbols 
% - Our approach: Multi-PAM symbols 
% - Complexity

% % joint source-channel coding scheme. 
% %  Constant sparsity 


% %%%%% Outline

% \section{Outline}



==> jsac/sysmodel.tex <==
\section{System Model}\label{sec:sysmodel}

We consider a feedback coding scheme with an AWGN forward channel and an AWGN feedback channel with noisy passive feedback. The goal is to transmit a message vector $\mathbf{u} \in \{0,1\}^K$ of length $K$ to the receiver using a total of $D$ independent channel uses \textit{i.e.,} the noise across the rounds is independent and identically distributed (i.i.d). This results in an overall coding rate of $R=\sfrac{K}{D}$. In this work, we consider symbol-by-symbol coding, where the block of $K$ bits will be mapped to one symbol. Hence, the terms block and symbol can be used interchangeably, and the number of rounds of communication for a rate $\sfrac{K}{D}$ code is $D$.

\begin{figure}[!htb]
% \vspace{-1em}
    \centering
 	\includegraphics[width=\linewidth]{figs/sysmodel.pdf}
 	\captionsetup{font=small}
 	\caption{Illustration of the $i^{\text{th}}$ round of communication for channels with feedback. The encoder takes as input the message bits $\mathbf{u}$ and the encoder output from previous rounds $x^{(i-1)}$, concatenated with the feedback from previous rounds $\Tilde{y}^{(i-1)}$, to compute $x_i$.}
    \label{fig:sysmodel}

\end{figure}

In the first round, the transmitter encodes the message block $\mathbf{u} \in \{0,1\}^K$ to a real-valued output $x_1 \in \mathbb{R}$ and transmits using the forward AWGN channel as
\begin{align}
    x_1 &= \phi(\mathbf{u}), \\
    y_1 &= x_1 + n_1,
\end{align}
where $\phi$ is the encoding function and $n_1 \sim \mathcal{N}(0,\sigma^2_{ff}) \in \mathbb{R}$ denotes the feedforward noise. The receiver then sends the noisy received symbol as feedback using the feedback channel as
\begin{equation}
    \Tilde{y}_1 = y_1 + \Tilde{n}_1,
\end{equation}
where $\Tilde{n}_1 \sim \mathcal{N}(0, \sigma_{fb}^2) \in \mathbb{R}$ denotes the feedback noise.


At round $i > 1$, the encoder $\phi$ computes the output $x_i$ using the input message bits $\mathbf{u}$ and the encoder outputs from previous $i-1$ rounds $x^{(i-1)} = \{ x_1, \dots, x_{i-1} \}$ and the feedback from previous $i-1$ rounds $\Tilde{y}^{(i-1)} = \{ \Tilde{y}_1, \dots, \Tilde{y}_{i-1} \}$ as 
\begin{equation}
    x_i = \phi \left(\mathbf{u}, x_1, \dots, x_{i-1}, \Tilde{y}_1, \dots, \Tilde{y}_{i-1} \right).
\end{equation}
% % where $x_i \in \mathbb{R}$, $x_{i-i}$ is the encoded symbol from round $i-1$ and $n_i + \Tilde{n}_{i-1}$ is the cumulative noise corresponding to forward and feedback transmissions from round $i-1$ computed as $n_i + \Tilde{n}_{i-1} = y_{i-1} - x_{i-1}$. 

% The transmitter then sends the encoded symbol over the forward channel as 
% \begin{equation}
%     y_i = x_i + n_i,
% \end{equation}
% where $n_i \sim \mathcal{N}(0, \sigma_{ff}^2) \in \mathbb{R}$ is the noise and $y_i \in \mathbb{R}$ is the received symbol. The receiver sends the new received symbol $y_i$ to the transmitter as feedback using the feedback channel as
% \begin{equation}
%     \Tilde{y}_i = y_i + \Tilde{n}_i,
% \end{equation}

% where $\Tilde{n}_i \sim \mathcal{N}(0, \sigma_{fb}^2) \in \mathbb{R}$ is the noise which is used for generating the next transmission $x_{i+1}$. 

At the end of $D$ rounds of communication, the decoder $\psi$ estimates the transmitted message vector $\hat{\mathbf{u}}$ using the received symbols from all $D$ rounds $\{ y_1, y_2, \dots, y_D \}$ as
% vector $\mathbf{y}^{(i)}$ and the received vectors from previous rounds $\{ \mathbf{y}^{(i-1)}, \dots, \mathbf{y}^{(2)}, \mathbf{y}^{(1)} \}$, to produce the new estimate $\hat{\mathbf{u}}^{(i)}$ given by
\begin{equation}
    \hat{\mathbf{u}} = \psi \left( y_1, y_2, \dots, y_D \right),
\end{equation}
where $\psi$ is the decoding function and $\hat{\mathbf{u}} \in \{0,1\}^K$. The objective is to design an encoder-decoder pair $\{\phi,\psi\}$ that minimizes the probability of error $\Pr\{\mathbf{u} \neq \hat{\mathbf{u}}\}$ for a given number of rounds $D$, under a sum power constraint of $\sum_{i=1}^D \mathbb{E}[|x_i|^2]\ \leq\ D$.
% We reiterate that the feedback sequence $\hat{\mathbf{u}}^{(i)} \in \{0,1\}^N$ is restricted to a binary sequence, making it  practical for resource-constrained settings and comparable to traditional HARQ schemes.  %as feedback using the noiseless feedback channel \begin{equation}  \Tilde{\mathbf{y}}^{(i)} = \hat{\mathbf{u}}^{(i)}. \end{equation}

% This process is continued until an error-free decoding or a maximum number of rounds $D$ is reached. The objective is to design a pair of encoder-decoder $\{\phi^{(i)},\psi^{(i)}\}_{i=1}^D$ that minimizes the probability of error $\Pr\{\mathbf{u} \neq \hat{\mathbf{u}}^{(D)}\}$ for a given maximum number of rounds $D$.

==> rebuttal.tex <==


% \onecolumn

\section*{Response to Reviewers' comments }

We thank the reviewers for their valuable and constructive feedback, which allows us to improve our paper. Below, we provide detailed responses to each of the comments provided by the reviewers. We revised the manuscript with the suggested changes highlighted so that the reviewers could easily see our modifications; we also conducted careful proofreading and corrected the typos, including those pointed out by the reviewers.

\subsection{Reviewer A}

\begin{enumerate}
    \item \textit{The message length considered in the paper is very small, i.e., $K=3$. It would be better to provide some results for a larger $K$.} 

    \medskip
    
    \textbf{Response.} Thank you for the suggestion. 
    \smallskip 
    
    $\bullet$ {\em Why $K=3$?} As a result of the curse of dimensionality, it is well known that the hardness of learning a code increases considerably with an increase in block length. Hence, instead of learning a longer blocklength, we propose keeping the blocklength short and treating a large block of information bits as independent sub-blocks of smaller blocklengths. For instance, GBAF~\cite{ozfatura2022all} uses a self-attention-based transformer to scale the block coding to length $51$. However, \lightcode achieves BLER superior to GBAF while using a code of length $3$ by treating a block of $51$ bits as $17$ independent sub-blocks of length $3$.
    \smallskip
    
    $\bullet$ {\em \lightcode trained with a larger blocklength $K$.\ } Following the suggestion, we ran experiments to train \lightcode with $K=6$ and  provide the results below. 

        \begin{table}[ht]
    \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{BLER} & Enc dimension & Dec dimension & \textbf{Total \# params} \\
    \hline
    $3.7 \times 10^{-4}$ & 32 & 32& $7.3 \times 10^3$ \\
    $7.2 \times 10^{-5}$ & 128 & 64 & $1.09 \times 10^5$ \\
    $2.4 \times 10^{-6}$ & 128 & 128 & $4.1 \times 10^5$ \\
    \hline
    \end{tabular}
    \captionsetup{font=small}
    \caption{BLER for K=6 at forward SNR of $-1.0$ dB and noiseless feedback.}
    \label{tab:bler_k_6_reb}
    \end{table}

We begin by comparing the performance of \lightcode for $K=6$ while maintaining the same encoder-decoder dimension used for $K=3$, which is $32$. From~\figref{fig:bler_3_9_noiseless}, the BLER of \lightcode trained with $K=3$ at a forward SNR of $-1.0$ dB and noiseless feedback is $4.5 \times 10^{-10}$. Hence, by transmitting $6$ bits as two sub-blocks, the BLER would be given by $1 - (1 - 4.5 \times 10^{-10})^2 = 9 \times 10^{-10}$. But, as seen from~\tabref{tab:bler_k_6_reb}, the BLER performance for \lightcode trained with $K=6$ and a hidden dimension of $32$ is orders of magnitude higher, $3.7 \times 10^{-4}$. Next, we increase the hidden dimensions to $128$, increasing the total number of parameters by $100 \times$, and the performance is still much worse than \lightcode trained with $K=3$.

\smallskip

We added the results for $K=6$ in the appendix of the revised manuscript in Appendix,~\secref{app:long_lightcode} on page 15. 

    \medskip
    
    % introduces a block coding with length $51$, using self-attention based transformer. In contrast, we argue that block coding in this regime does not add value and is even detrimental in case of limited computational complexity. Instead, we propose treating a larger code block as a collection of smaller sub-blocks of length $K=3$ and independently encoding each sub-block, similar to the recent work Robust Coding~\cite{kim2023robust}, essentially implementing a symbol by symbol coding. For example, to transmit $6$ bits, we transmit encode the first $3$ bits into symbol 1 and next 3 bits into symbol 2. More details and results for the same are provided in~\secref{sec:noisy} on page 10. 
    
%    {\color{red} This paragraph is a little bit all over. Doesn't read smoothly. Modularize ideas -- (1) Here's the results for K=6. (2) ... (3)... Also, we're saying `to transmit 6 bits, we transmit 3 bits (x2). So what? Is that better than learning to transmit 6 bits all together? Transmitting 3 bits (x17) using our scheme is better than transmitting 51 bits using GBAF? Assume that the reader forgot about our paper (it's probably the case, actually). We shall assume that the reader forgot everything; the responses should thus be self-contained. For example, `more details and results are provided on page 10' is not very satisfying. Do you wanna say that something along the line of ... even though our K is small, we achieve very good results?} 

    % \qquad 1. For completeness, we provide the performance for $K=6$ at different complexity of the encoder-decoder at forward SNR = $-1.0$ and noiseless feedback. 
    
%    {\color{red} What's the interpretation? This is worse than the results for $K=3$ (x2)? }

 %   \textcolor{blue}{Updated; needs to be reviewed.}

    

    \medskip

    \item \textit{Are the coding schemes considered in Figs. 5-7 have different message lengths $K$?} 

    \medskip

    \textbf{Response.}
    Thank you for raising this important point. 

    \smallskip 

    $\bullet$ Fig. 5 and Fig. 7: The lengths considered for each coding scheme for Fig. 5 and Fig. 7 are listed below. % {\color{red}Is this table relevant to all three figures?} \textcolor{blue}{This is relevant for figures 5,7.}

    \begin{table}[!ht]
    \centering
    \begin{tabular}{lc}
    \hline
    \textbf{Scheme} & \textbf{ Message length $K$} \\
    \hline
    Deepcode & $50$ \\
    DEFC & $50$ \\
    DRFC & $50$ \\
    AttentionCode & $50$ \\
    \gn & $3$ \\
    \pb & $3$ \\
    Robust Coding & $3$ \\
    GBAF & $3$ \\ % I removed x17 here. Sure
    \lightcode & $3$ \\    
    \hline
    \end{tabular}
    \captionsetup{font=small}
    \caption{Block lengths of different coding schemes.}
    \label{tab:block_lengths_reb}
    \end{table}

     The blocklength for some of the schemes considered in Fig. 5 and Fig. 7 is $K=50$, which is larger than the length $K=3$ considered for the rest of the schemes, including \lightcode.  Note that while GBAF uses a blocklength of $51$, the BLER in~\cite{ozfatura2022all} was reported for the sub-block of $3$ bits. While the comparison against the schemes of different blocklengths is not fair, to maintain consistency, we followed the same methodology followed in the current state-of-the-art results, including GBAF~\cite{ozfatura2022all} and Robust Coding~\cite{kim2023robust}.
     

     \medskip 
     $\bullet$ Fig. 6: For a fair comparison against schemes with block length $K=50$, we refer to the results in~\figref{fig:bler_3_9_noiseless_51} where we compute the BLER for longer block length by treating a block of $L=51$ bits as $17$ independent sub-blocks of length $K=3$, encoding $3$ bits at a time. Thus we follow a symbol-by-symbol coding by encoding each sub-block of $3$ bits into $1$ symbol. The BLER of a blocklength $51$ can be computed as
     \begin{equation}
         p_{51} = 1 - (1-p_3)^{17},
     \end{equation}
     where $p_3$ is the BLER of length $K=3$ scheme. Hence, the BLER of length $51$ is higher than the BLER of length $3$. But from~\figref{fig:bler_3_9_noiseless_51}, we can see that this is still significantly smaller than the baselines with codeblock length $50$, demonstrating the superior performance of \lightcode even at longer lengths. 

     We added a detailed discussion on the same in the revised manuscript in~\secref{sec:long_length} on page 10. 

     % {\color{brown} Was this not clear in the paper? if so, we can add a sentence or two describing this mismatch etc and say we added this in the revised manuscript.} 

     
     % Because of symbol by symbol coding, there is a performance drop for \lightcode from length $3$ to $51$. 
     
     % {\color{red}$\leftarrow$ This statement is not clear. `performance drop' is not clear. You mean BLER? Be specific. Also, the term symbol-by-symbol coding needs to be clarified.} \textcolor{blue}{Updated; needs to be reviewed.}
     % But the BLER is still significantly lower than the baselines with codeblock length $50$, demonstrating the superior performance of \lightcode even at longer lengths.
     % {\color{red} Modularize the key ideas better. For example, we might wanna separate the discussion on Figure 6 and Figures 5/7.}
    % \textcolor{blue}{The above is the discussion for Fig 5, using the results from Fig 6 for longer block lengths (using 51 = 3x17 approach). For Fig 7, we did not include the results for longer blocklengths in the paper.}
    
    \medskip

    \item \textit{The authors identify some similarities between \lightcode and \pb. If both schemes are similar, why \lightcode can achieve better BLER than \pb in the low SNR regime?} 

    \medskip
    
    \textbf{Response.} We identify the similarity between \lightcode and \pb in terms of power allocation across positions and their behavior during initial rounds of communications. However, a key difference between \lightcode and \pb is the non-linear nature of the codewords with respect to the input message. As described in \secref{sec:interpret} on page 13 and shown in~\figref{fig:linear_reg} on page 14, while the behavior of \lightcode can be approximated by a linear scheme in the initial rounds, it becomes increasingly {\em non-linear} in the later rounds. % {\em non-linearity} becomes essential in later rounds, limiting the performance possible by a linear scheme such as \pb.
     We hypothesize that this non-linearity contributes to the improved BLER in the low-SNR regime. 
    %{\color{red}There are two key messages? One is regarding the power allocation. The other is initial rounds vs. later round? Let's use numbers to be clear about this.}
    \medskip

    \item \textit{Please provide the formal definition of throughput.} 

    \medskip
    
    \textbf{Response.} Thanks for the suggestion. We now added a formal definition for throughput in bits/sec for a given rate in Section~\ref{sec:comp_throughput} on page 12. 

    \medskip

    \item \textit{It would be better to analytically quantify the complexity of the proposed schemes. For example, how does the complexity of \lightcode scale with the target BLER?} 

    \medskip
    
    \textbf{Response.} %Analytically quantifying the complexity of deep learning based channel coding schemes with respect to target BLER would be very nice but is highly non-trivial and an open problem. We instead conduct an empirical study to analyze the trade-off in complexity vs performance of \lightcode.
%
    While analytically quantifying the complexity of deep-learning-based channel coding schemes with respect to target BLER would be very interesting, it is highly non-trivial and a widely open problem. Thus, we instead conduct an empirical study to analyze how the complexity of \lightcode scales with the target BLER. 

    \medskip
    
    Empirically, we observed that reducing the complexity of the decoder while maintaining the same complexity for the encoder provided the best trade-off in performance vs complexity. In this experiment, we vary the target BLER and find the required encoder-decoder dimensions for a rate $\sfrac{3}{9}$ code at a forward SNR of $-1.0$ dB and a noiseless feedback channel. The results for the same are shown in~\tabref{tab:bler_tradeoff} and~\figref{fig:complexity_tradeoff} and included in the revised manuscript in~\secref{sec:comp_throughput} on page 12.

    \medskip
    
    % for $K=3$, decreasing the hidden dimension of encoder below $32$ is resulting in a significant drop in performance. 
   % {\color{red} $\leftarrow$ How is this answer related to the question? (Also K=3 is not an important aspect here.) We'd better get to the relavent answer directly. In the experiment, we vary the target BLER and empirically find the required enc-decoder dimensions... and the results are shown in Figure 12. Note that we have enc-dec pairs. We maintain the encoder complexity the same and find the required decoder complexity.. (Why is the bottom row bold? Here why is the encoder dimension 16?)} \textcolor{blue}{Updated; needs to be reviewed.}
    % Hence to reduce complexity, it is recommenced to reduce the hidden dimension of decoder. Below we provide the complexity vs performance trade-off for rate $\sfrac{3}{9}$ \lightcode with noiseless feedback at a forward SNR of $-1.0$ dB. We maintain the encoder complexity the same and reduce the decoder complexity by decreasing the hidden dimension. 

%    2. Analytical study: 

    \begin{table}[!ht]
    \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{BLER} & Enc hidden dimension & Dec hidden dimension & \textbf{Total \# parameters} \\
    \hline
    $4.5 \times 10^{-10}$ & 32 & 32 &$7.3 \times 10^3$ \\
    $3.4 \times 10^{-9}$ & 32 & 16 &$4.7 \times 10^3$ \\
    $5.2 \times 10^{-9}$ & 32 & 12 &$4.3 \times 10^3$ \\
    $2.8 \times 10^{-8}$ & 32 & 8 &$3.9 \times 10^3$ \\
    % $\mathbf{1.3 \times 10^{-7}}$ & \textbf{16} & \textbf{32} &$\mathbf{5.9 \times 10^3}$ \\
    
    \hline
    \end{tabular}
    \captionsetup{font=small}
    \caption{Complexity vs BLER (total number of parameters) performance trade-off for rate $\sfrac{3}{9}$ code at a forward SNR of $-1.0$ dB and noiseless feedback. }
    \label{tab:bler_tradeoff}
    \end{table}
    \end{enumerate}


\begin{figure}[!htb]
    \centering
 	\includegraphics[width=0.6\linewidth]{figs/complexity.jpg}
 	\captionsetup{font=small}
 	\caption{Complexity (total number of parameters) vs. BLER performance trade-off for rate $\sfrac{3}{9}$. Encoder complexity is maintained the same while decoder complexity is reduced to decrease the number of parameters. The change in BLER is almost linear in the log scale with respect to the number of parameters. 
  % {\color{red}Besides, yes, more parameters - better BLER, is there anything else we can say about the trade-off? like linear scaling (which is obviously not the case here)} 
  % \textcolor{blue}{I think we can something like the trade-off is linear with respect to BLER in log scale.}
  }\label{fig:complexity_tradeoff}
% \vspace{-1em}
\end{figure}
\subsection{Reviewer B}
   %  {\color{red}Did Reviwer B have no other comments? They are all quite minor points.}\textcolor{blue}{Yes, he had almost nothing negative to say and gave a score of 9.}
    % {\color{brown}Grammar - pointing. pointing out. 1 and 2}
    \begin{enumerate}
    \item \textit{Some words are unnecessarily indented, such as "where" after (6).}  

    \medskip
    
    \textbf{Response.} Thank you for the suggestion. We corrected the indentation throughout the paper.


    \medskip
    
    \item \textit{Spelling and capitalization should be checked in places such as the first word in Section V.A.} 

    \medskip
    
    \textbf{Response.} Thank you for pointing out the typos. We fixed the capitalization and spelling throughout the manuscript. 


    \medskip
    
    \item \textit{There seems to be an accent mismatch for the author name in [4], Nakiboglu, that is widely used in the manuscript. Different letters are accented in the text and in reference; the reference seems to be the correct one.} 

    \medskip
    
    \textbf{Response.} Thank you for bringing the discrepancy to our notice. We fixed the accent on the paper to match the style in reference. 

    \end{enumerate}


\subsection{Reviewer C}

    \begin{enumerate}
    \item \textit{In Section V.A., the authors claim that linear estimators are suboptimal. Will this claim hold in the case of Gaussian modulation, or is it just an artifact of PAM?} 

    \medskip
    
    \textbf{Response.} It is an artifact of PAM. For the problem of transmitting a Gaussian source under an MSE distortion, linear estimators are optimal as shown in~\cite{gallager2009variations}. However, the problem of transmitting a {\em discrete symbol} (e.g., PAM) to minimize the {\em decoding error} is inherently different from minimizing the MSE. This is because equal distance from the decoding decision boundary does not translate into the same error, making the behavior non-linear. For example, consider transmitting a BPSK symbol $\theta \in \{-1,+1\}$ over an AWGN channel $y = \theta + z$, where $z \sim \mathcal{N}(0,1)$. The optimal decoder would map $y \ge 0$ to $\hat{\theta} = +1$. Thus, if $\theta = 1$, the receiver can tolerate any positive noise without making a decoding error. On the other hand, even a small negative noise will translate into a decoding error.
    
    \medskip

    Hence, while linear schemes such as SK and GN are suited/optimal for Gaussian sources, the optimality does not translate to discrete symbols like PAM, and the performance can be improved by adapting non-linear schemes. 
    
    %Whereas any negative error, despite having the same magnitude, will result in a decoding error. <- what do you mean by 'error'? Not all negative noise will translate to a decoding error. 
    % Hence, we see this as a limitation of PAM used in SK and GN schemes.
   % {\color{red} $\leftarrow$ This conclusion is not justified. Needs a bit more explanation. Sth like SK/GN optimized for Gaussian not suitable for PAM .... or linear schemes SK and GN are not suitable for PAM... we would like to provide a succinct but self-contained explanation. }\textcolor{blue}{Updated; needs to be reviewed.}


    \medskip
    
    \item \textit{In the presented numerical results (Fig. 6 and further), one can observe an error-floor effect. Most NN-based solutions face this issue. I kindly suggest the authors elaborate on this effect.}
    \begin{enumerate}

        \item[(a)] \textit{Is it the effect of training? Smaller probabilities of error result in the fact that errors become rare, and the gradient-descent algorithm becomes inefficient.}

        \item[(b)] \textit{Is it the effect of the numerical precision of weights?}

    \end{enumerate}

    \medskip
    
    \textbf{Response.} Thank you for raising this discussion. As rightfully pointed out, all existing deep-learning-based coding schemes, including \lightcode, show a saturation or error floor in high-SNR regions. We think the main reason for this behavior is the difficulty of training the decoder in the high SNR region, where the error events are extremely rare, corresponding to (a), the reviewer's first point. For instance, while training in the regime of BLER $10^{-9}$, most of the training batches (batch size $10^5$) are error-free and do not provide sufficient guidance for the gradient descent to learn useful information. We now added a discussion on this in~\secref{sec:comparison} on page 10. 
    
    \medskip

    Regarding (b), the reviewer's second point, we currently use a \texttt{float32} format to represent the weights and gradients, which can reliably represent values up to $10^{-38}$, and hence do not suspect the precision of weights being a reason for the saturation at high SNR. 


    \medskip
    
    \item \textit{In Table V, the authors consider the simulated throughput of different decoding schemes. Is it possible to make the same estimates for «classical» decoders, including the proposed PowerBlast?} 

    \medskip
    
    \textbf{Response.} We note here that comparing throughputs for classical schemes against deep-learning-based schemes is not straightforward and depends heavily on the implementation. Our implementation of \lightcode is done using \texttt{PyTorch} libraries, whereas \pb and other classical schemes were implemented using \texttt{NumPy} libraries. Further, a major computational bottleneck for the classical schemes is the necessity for demodulation after each round, the speed of which is heavily influenced by the implementation methodology. Hence, we restrict our comparison to the family of deep learning codes, where the latency primarily originates from the architecture complexity and the total number of parameters, and a fair comparison is feasible. 
    
    \smallskip 
    
    However, it is clear that the total number of numerical operations in classical schemes is significantly lower than that of deep-learning-based schemes, and we acknowledge that the throughput of classical schemes can be significantly higher than that of any deep-learning-based schemes. 

    \smallskip 
    
    We added a detailed discussion on these aspects in the revised manuscript in~\secref{sec:comp_throughput} on page 12.
    
    % {\color{brown} Q. Would you like to mention this in the revised paper? If so, we'll say we added this discussion in the revised manuscript.}
    
    % We restrict our focus to deep-learning-based schemes, among which \lightcode shows significantly lower complexity and higher throughput. 

    % Why DL only. 

    % PowerBlast * Number of operations/flops? To process a single bit, we need single multiplication, and Z demodulation. 
    % LightCode -- Processing using neural networks 

    % * numpy implementation / demodulation - sort / slow. Based on our implementation, here are the numbers. But can probably be optimized further. 
    % For classical schemes, SK, GN, and \pb have the same complexity and we measure the compute time in CPU mode. 

    % \begin{table*}[!ht]
    % \centering
    
    % \begin{tabular}{lcc}
    % \hline
    % \textbf{Scheme} & \textbf{ Enc (CPU)} & \textbf{ Dec (CPU)} \\
    % \hline
    % GBAF~\cite{ozfatura2022all} & $ 1.6 \times 10^5 $ & $ 1.7 \times 10^6 $ \\
    
    % Robust Coding~\cite{kim2023robust} & $ 2.0 \times 10^5 $ & $  7.6 \times 10^4 $\\
    
    % \lightcode (ours) & $\mathbf{1.5 \times 10^6}$  & $\mathbf{1.3 \times 10^7 }$ \\

    % SK / GN / \pb & $6.3 \times 10^6$  & $6.5 \times 10^5 $ \\
    
    % \hline
    % \end{tabular}
    % \captionsetup{font=small}
    % % \caption{Throughput (symbols/sec) comparison. Rate $\sfrac{3}{9}$ \lightcode achieves up to $ 10 \times $ higher decoding throughput compared to GBAF and up to $171 \times$ higher decoding throughput in CPU mode compared to Robust Coding.}
    % \label{tab:sk_inference}
    % % \vspace{-1em}
    % \end{table*} 

    \medskip    

    \item \textit{Is it possible to add some discussion about the channel capacity? [e.g., 1]. Adding some references to the plots would be nice.} 

    \medskip
    
    \textbf{Response.} Thanks for the reference. We added references in the plots in Fig. 5, 7 to indicate the channel capacity, making the comparison easier. As we consider memoryless channels, the capacity does not increase as we incorporate feedback. 

    \medskip

    \item \textit{I did not understand the nature of~\figref{fig:deepcode_scaling} and the corresponding discussion. The reduced batch size would result in a lower required learning rate and a longer training time.} 

    \medskip
    
    \textbf{Response.} 
    
    $\bullet$ {\em Nature of~\figref{fig:deepcode_scaling}}: Our main takeaway from~\figref{fig:deepcode_scaling} is to show that a very large batch size is required to achieve the best possible performance. By limiting to a lightweight design, \lightcode makes this possible and supports a batch size of $>10^5$  whereas the baseline code GBAF can only support a batch size of $<10^4$ on a \texttt{NVIDIA GeForce RTX 4090} GPU with a RAM of 24 GB.
    \smallskip 
    
    $\bullet$ {\em Learning rate/training time}: We would like to clarify that for each batch size, hyperparameters such as learning rate have been optimized, and the model is trained until saturation to ensure the best possible performance. We have added these details to the discussion in~\secref{sec:scaling} on page 12. Further, we use a learning rate scheduler to gradually decay the learning rate to a very small value, thus minimizing the variance in performance because of differences in the learning rate, as mentioned in~\secref{sec:training}.
     
     
     % the best performance achievable by the \lightcode scheme is dependent on the batch size used and the performance improvement with respect to batch size saturates around a very large batch size of $5\times10^4$. Further, the extremely low complexity of \lightcode makes it feasible to train the model with such a large batch size. \\
    
    
    
    
    % We first clarify that we train the model for same number of epochs in both cases. Further, we experimented with various hyperparameter settings to optimize the result for each batch size and empirically conclude that the best performance is achieved at a sufficiently large batch size, which helps in bringing the power distribution close to Schalkwijk-Kailath. The key takeaway of Fig. 8 is to systematically study the scaling laws and show that given a sufficiently large batch size, the performance of a simple symbol-by-symbol scheme can match or exceed the performance of much more complex GBAF block coding scheme. 

    \medskip

    \item \textit{I also found some minor issues that can be fixed:} 

    \begin{enumerate}
        \item Please double-check the bib file. Some capital letters are missing (e.g., reference [4]).
        \item Section V.A. starts with a lower-case letter.
    \end{enumerate}

    \medskip
    
    \textbf{Response.} Thank you for pointing out the typos. We have now fixed the issue of capitalization in references and Section V.A.
    

    \end{enumerate}


\subsection{Reviewer D}

   \begin{enumerate}
        \item \textit{ The system set-up does not make it clear that the noises are i.i.d. in time.} 

        \medskip
        
        \textbf{Response.} Thank you for pointing this out. We added a statement in \secref{sec:sysmodel} on page 2 to make this clear.

        \medskip
    
        \item \textit{I do not understand the high SNR performance improvements of PowerBlast.  Can you add more explanation?  It is a dramatic improvement, and I can not figure out why this happens given the similarities to SK and GN.} 

        \medskip
        
        \textbf{Response.} 
        % Thanks for raising this important discussion. The key difference between \pb and SK/GN schemes is the focus of \pb on performance in non-asymptotic regime. To simplify the error analysis and show the exponentially decaying error, SK uses a minimum-variance unbiased estimator (MVUE) after round 1~\cite{ben2017interactive} and communicates the noise $Z_0$ from round 1 over the remaining $D-1$ rounds~\cite{gallager2009variations}. From~\cite{ben2017interactive}, it is seen that the effective SNR after $D$ rounds is given by $S(1+S)^{D-1}$ using an MVUE estimator whereas $(1+S)^{D} - 1$ when using LMMSE estimator. While the effective SNR converges to the same value for the asymptotic case of $D \to \infty$, for finite rounds of communication, the difference in effective SNR becomes significant. 
        
        \smallskip
        
        \textbf{\pb vs. SK:} The key difference between \pb and SK is in the last round of communication, where \pb shifts to a discrete symbol scheme, as seen in line 13 of~\algref{alg:PB}, by taking advantage of the high effective SNR over the $D-1$ rounds \textit{i.e.,} the noise variance is much smaller than the distance between adjacent PAM symbols. Hence, it is beneficial to now transmit the error in the PAM constellation index, which $\in \{-1, 0, 1\}$ with very high probability, and results in a much lower probability of error.  

        \smallskip

        \textbf{\pb vs GN:} The key difference between \pb and GN is in the choice of information transmitted after round 1. GN communicates and refines the noise from round 1 $N_1$, starting round 2, as seen in line 4 of~\algref{alg:GN}, whereas \pb transmits and refines the error in LMMSE estimate of $\Theta$, as seen in line 4 of~\algref{alg:PB}. It is seen from~\cite{ben2017interactive} that the effective SNR (in linear scale) after $D$ rounds is given by $S(1+S)^{D-1}$ for GN. In contrast, the effective SNR for \pb which uses LMMSE after round 1 is given by $(1+S)^{D} - 1$. While the difference in effective SNR becomes negligible for large $D$, it can be significant when operating for a finite number of rounds, resulting in the superior performance of \pb.
        
        \smallskip
        
        We now added a detailed explanation on the same in~\secref{sec:pb} on page 5 in the revised manuscript.
        
        % We attribute the impressive gains of \pb over SK and GN to the choice of estimator after round 1. To simplify the error analysis, the estimator after round 1 in SK uses MVUE estimate of the transmitted symbol $\hat{\Theta}_1$, as seen in line 3 of~\algref{alg:SK}~\cite{ben2017interactive} and also in Eq. 15. This assumption is necessary in showing an exponentially decaying error exponent for SK but is not optimal for minimizing the decoding error after finite rounds of communication. It is seen from~\cite{ben2017interactive} that the effective SNR (in linear scale) after $D$ rounds is given by $S(1+S)^{D-1}$ using an MVUE estimate whereas $(1+S)^{D} - 1$ when using LMMSE estimate, where $S$ is the SNR in linear scale for forward AWGN channel. While the effective SNR converges to the same value for the asymptotic case of $D \to \infty$, the difference in effective SNR becomes significant for finite rounds of communication. Further, instead of refining the error in estimate, GN aims to communicate the noise realization from round 1~\cite{gallager2009variations}, as shown in line 4 of~\algref{alg:GN}, which is the strategy developed by Elias~\cite{Elias1956ChannelCapacity} to communicate a Gaussian random variable. While this a suitable strategy for achieving an exponentially decaying error exponent, this also does not optimize for the BLER performance after finite rounds of communication, as seen in~\figref{fig:bler_gn_vs_pb}. Hence, by using the LMMSE estimate and iteratively refinig the error in estimate, \pb achieves a superior performance for a given finite number of rounds of communication.
        
        % {\color{brown} Before you bring up the term LMMSE estimator, mention that Powerblast uses the LMMSE estimator (it's not written in the description). Also, what about the discussion on GN?}\textcolor{violet}{Updated; needs to be reviewed.}
        % {\color{red} `transmits the noise using the remaining rounds' this is not quite correct - as the transmission at each round is not the noise itself. I'd rather write something like `aims to communicate the noise $Z_0$ over the remaining D-1 rounds'} 
        % This assumption is valid and does not make a difference for the asymptotic case of $N \to \infty$. 
        % {\color{red} does not make a difference on what? what do you mean by a valid assumption? what is a valid assumption?} But for finite rounds of communication, the difference in effective SNR becomes significant and using an LMMSE estimator in \pb provides a noticeably better effective SNR at the end of $N$ rounds of communication. {\color{red}I'm a bit confused- as LMMSE estimator is unbiased}
        
        \medskip 
        
        % Hence, in summary, by using the LMMSE estimate and transmitting the error, instead of using MVUE estimate and transmitting the noise, \pb achieves a much superior performance for a given finite number of rounds of communication. We now added a discussion on the same in \secref{sec:pb} on page 5.\textcolor{blue}{Updated; needs to be reviewed.}

        \medskip
        
        \item \textit{I find the \lightcode architecture descriptions too vague.  This is a problem because it will affect the ability of others to understand and build upon this work.} 

        \medskip
        
        \textbf{Response.} Thank you for pointing this out. We expanded the description of the model architecture and training methodology in~\secref{sec:deepcode} on page 8 to provide additional details. Further, we intend to release the source code and the steps to reproduce the results with the camera-ready version of the paper.

        \medskip

        \item \textit{Ref \cite{shao2023attentioncode}, \cite{ozfatura2022all} have an unclear explanation issue, and it makes it hard to digest the GBAF comparisons.} 

        \medskip
        
        \textbf{Response.} 
        \smallskip 
        
        $\bullet$ {\em More details on the baseline schemes.\ } % To keep the work concise, we limited the discussion on the details on [25], [26]. But 

        \smallskip 
        We now added more details on AttentionCode~\cite{shao2023attentioncode} in~\secref{sec:gbaf} paragraph 1 on page 6, and the details on GBAF~\cite{ozfatura2022all} can be found in paragraph 2. In summary, the following are the key differences across the baseline architectures considered. DeepCode~\cite{kim2018deepcode} introduced the idea of using RNN architecture to model the dependencies across rounds and positions to design neural codes for channels with feedback. AttentionCode~\cite{shao2023attentioncode} improved this design by replacing RNNs with a more powerful sequence-to-sequence model, a self-attention-based transformer, to improve the modeling of temporal dependencies. GBAF~\cite{ozfatura2022all} improved this further by leveraging the transformer architecture to explicitly perform block coding across the bit positions and achieving the current state of the art regarding BLER. 

        \medskip

        $\bullet$ {\em How is \lightcode different from the schemes above?} % We would like to highlight three key differences. 

        \smallskip 
        A key difference between \lightcode and the baseline schemes above is the {\em code length}: while the schemes above % In contrast to the above schemes which 
        use a block length of $K=50$, \lightcode learns a code of length $K=3$. 
% 

        \smallskip 
        Although it was previously believed that longer blocklengths improve reliability (coding gain), we show this is not necessarily true. The reliability of \lightcode, measured in the BLER for $K=51$ by independently encoding a sub-block of 3 bits at a time ($\times$ 17), is superior or on par with the state-of-the-art GBAF as seen from~\figref{fig:bler_3_9_noiseless} and ~\figref{fig:bler_3_9_noiseless_51}.

%
%        \smallskip 
        We attribute this improvement to two factors. The first is reduced complexity. As we considered a shorter code length, we were able to reduce the complexity of the encoder-decoder architecture by a factor of $10 \times $; specifically, we eliminate the transformer module used in GBAF for block coding and further reduce the complexity of feature extractor,
        % {\color{brown} we removed a transformer...  and simplifies the feature extractor ... }
        using simple feed-forward and skip connections as seen in~\figref{fig:feature_extractor}. Second, the shorter code length and lightweight architecture allowed us to train \lightcode with an extremely large batch size of $10^5$, which is more than $10 \times$ larger than
        % {\color{brown} how many times XX} times larger than 
        the maximum batch size possible for GBAF codes. %which was made possible as we considered a shorter code and lightweight architecture. % As a result, \lightcode achieves a extremely low BLER and scales the performance to longer blocklengths by independently encoding a sub-block of 3 bits at a time, achieving superior performance compared to the state-of-the-art GBAF as seen from~\figref{fig:bler_3_9_noiseless} and ~\figref{fig:bler_3_9_noiseless_51}.

        \smallskip 
        We find it surprising that a code trained for $K=3$ is at least as reliable as one trained for $K=50$. 
        On the one hand, our results suggest that the learning-driven codes may not fully utilize the achievable coding gain. On the other hand, it raises an important question about the fundamental gain achievable by coding for non-linear feedback codes, a question that remains widely open.  

        \smallskip

        We now added a discussion on the same in~\secref{sec:arch} on page 8.
        
        
        % {\color{brown} Any changes to be copied to the main text?}

        % \textcolor{blue}{Sure .. I will cross verify this and copy after we finalize the rebuttal responses.}
        
        % The important differences between DeepCode and [25], [26] have been highlighted in~\secref{sec:gbaf} for reference. 
        %{\color{brown} Throw a few keywords for the difference?}{\color{violet} Updated; needs to be reviewed.} 
        
        % Also did you mean Deepcode or Lightcode?}
  %      {\color{red} Do you think we can highlight some key aspects so that this reviewer can `digest' the GBAF comparisons? It's okay to copy and paste the descriptions in the main text. } \textcolor{blue}{Actually, I think we provided sufficient details in ~\secref{sec:gbaf}. But I can try adding more details. }
        
        \medskip

        \item \textit{The plots in Section 7 are very difficult to read and understand.  I like that exhaustive simulations have been done, but there are just too many things happening in the plot.  It is even harder to understand when it is in black-and-white.  The current text explaining the figures is rather short.  I would adjust the explanation to make them more explanatory.  I would highlight the key takeaway from the figure and remove curves that obscure this key takeaway.} 

        \medskip
        
        \textbf{Response.} Thank you for your suggestions. We agree that the figures are a little crowded and have updated the~\figref{fig:bler_3_9_noisy} on page 11 to make it more readable. Specifically, we removed the results for noiseless feedback and plotted only the results for noisy feedback to reduce the total number of plots and make the comparisons easier to observe. 

        \medskip
        
        Further, in~\figref{fig:bler_3_9_noiseless_51} on page 11, we removed the results for $L=99$ and $L=300$, as they can be computed analytically using Eq. 20. Instead, we now added results for $L=51$ to make a direct comparison against baselines with $K=50$ blocklengths.
        
        % {\color{red} added results for L=51? you mean removed? } \textcolor{blue}{We previously had results for $L=99$ but we removed them. But now added results for $L=51$ to make the comparison against baselines fairer.} {\color{brown} ok - can you describe the overall changes?}

    \end{enumerate}

    \twocolumn

==> related_works.tex <==
\section{Related Works}\label{sec:rel_works}
In this section, we briefly review the current state of coding for channels with passive feedback. Existing feedback communication schemes can be broadly classified into two categories. The first is human-crafted codes that are carefully designed to improve the error correction probability after each round in a sequential manner. The seminal work of Schalkwijk-Kailath \cite{schalkwijk1966coding_p1,schalkwijk1966coding_p2} used a fixed block length coding scheme with $2^K$-ary PAM constellation, $K$ is block length. It demonstrated that feedback could result in a second-order exponential decay of decoding error for all transmission rates less than capacity. Later, Zigangirov \cite{zigangirov1970upper} demonstrated that for the case of finite bandwidth, the doubly exponential bound can be replaced by $K^{\th}$ order exponential bounds for asymptotically large lengths. Similar lines of work can be found in \cite{martins2008coding,gallager2009variations,chance2011concatenated,kim2007gaussian,ben2017interactive}. While these schemes promise impressive theoretical guarantees in terms of performance, they quickly suffer from numerical precision issues in practice, as the length increases. Hence, commonly used schemes in practice are still limited to ARQ and HARQ, which do not fully utilize the capabilities of the available high-fidelity noiseless feedback channel, as demonstrated by CE-HARQ\cite{ankireddy2023compressed}.

% Commonly used schemes in practice are Automatic Repeat Request (ARQ) and Hybrid Automatic Repeat Request (HARQ), which utilize simple 1-bit feedback from the receiver to indicate success by acknowledgment (ACK) or a failure by negative acknowledgment (NACK). These schemes are primitive and do not  


Recent advances in machine learning and deep learning enabled the creation of a new line of work in the area of channel coding by leveraging the expressive power~\cite{raghu2017expressive} of deep neural networks. Several works explored various approaches to improving the performance of channel codes for point-to-point channels ranging from augmenting classical decoder with learnable parameters~\cite{nachmani2016learning, nachmani2018deep, ankireddy2023interpreting, hebbar2022tinyturbo} to creating novel neural network architectures based neural encoders and decoders~\cite{hebbar2023crisp, hebbar2024deeppolar} and improving the code design using sequential models~\cite{li2021learning,ankireddy2024nested}. Another line of work explored coding for channels with feedback, where deep learning techniques were used to design new encoding and decoding schemes by taking advantage of the high-capacity feedback channel. In this aspect, the seminal work by Kim et al. Deepcode~\cite{kim2018deepcode} modeled both encoder and decoder functions as recurrent neural networks (RNNs) to process a bit stream in a sequential manner to directly minimize the end-to-end transmission error over an AWGN channel. This was further extended in deep extended feedback (DEF) codes~\cite{safavi2021deep} to introduce modulation to increase spectral efficiency and also to use more power sequential models such as long short-term memory (LSTM) architecture to model the dependency over higher rounds of communication. Further, in~\cite{mashhadi2021drf}, deep SNR-robust feedback (DRF) codes were introduced, which explored the generalization of Deepcode and DEF codes to multiple SNRs using SNR-aware attention and curriculum training with batch size scheduling. Later, a new level of performance was achieved by replacing RNNs and LSTM models with self-attention based transformer models in AttentionCode~\cite{shao2023attentioncode}. More recently, generalized block attention feedback (GBAF) codes were introduced in~\cite{ozfatura2022all}, which is currently the state-of-the-art deep learning-based feedback code with passive feedback. GBAF uses a self-attention mechanism to do block coding across the codeword, introducing dependencies across the positions and improving the decoding performance by an order of magnitude over the previous deep learning-based feedback codes. This clearly demonstrates that a new level of error-correcting performance for feedback codes can be achieved by leveraging advances in deep learning. In another work, Robust Coding~\cite{kim2023robust} focused on designing codes for channels with noisy feedback using bi-directional attention-based decoding architecture. But these state-of-the-art solutions come at an increasingly high computational cost, potentially exponentially more complex compared to human-crafted codes, and motivate us to look for low-complex solutions. We also note that further improvements can be achieved by using active feedback~\cite{chahine2022inventing,ozfatura2022feedback}, but we limit ourselves to passive feedback in this work. 
